Influences on LLM Calibration: A Study of Response Agreement, Loss Functions, and Prompt Styles

Calibration, the alignment between model confidence and prediction accuracy, is critical for the reliable deployment of large language models (LLMs). Existing works neglect to measure the generalization of their methods to other prompt styles and different sizes of LLMs. To address this, we define a controlled experimental setting covering 12 LLMs and four prompt styles. We additionally investigate if incorporating the response agreement of multiple LLMs and an appropriate loss function can improve calibration performance. Concretely, we build Calib-n, a novel framework that trains an auxiliary model for confidence estimation that aggregates responses from multiple LLMs to capture inter-model agreement. To optimize calibration, we integrate focal and AUC surrogate losses alongside binary cross-entropy. Experiments across four datasets demonstrate that both response agreement and focal loss improve calibration from baselines. We find that few-shot prompts are the most effective for auxiliary model-based methods, and auxiliary models demonstrate robust calibration performance across accuracy variations, outperforming LLMs' internal probabilities and verbalized confidences. These insights deepen the understanding of influence factors in LLM calibration, supporting their reliable deployment in diverse applications.

==> tables/deberta_nq_large.tex <==
\begin{table*}[h!]
\centering
\scriptsize
\renewcommand{\arraystretch}{1.1} % Adjust row height for readability

\begin{tabular}{l@{\hspace{0.19cm}} l@{\hspace{0.19cm}}|l@{\hspace{0.19cm}}l@{\hspace{0.19cm}}l@{\hspace{0.19cm}}l@{\hspace{0.19cm}}|l@{\hspace{0.19cm}}l@{\hspace{0.19cm}}l@{\hspace{0.19cm}}l@{\hspace{0.19cm}}|l@{\hspace{0.19cm}}l@{\hspace{0.19cm}}l@{\hspace{0.19cm}}l@{\hspace{0.19cm}}|l@{\hspace{0.19cm}}l@{\hspace{0.19cm}}l@{\hspace{0.19cm}}l}
% \rowcolor{gray!30}
\toprule
 & \multirow{2}{*}{\textbf{Method}} & \multicolumn{4}{c}{\textbf{Verb.}} & \multicolumn{4}{c}{\textbf{Zero-shot}} & \multicolumn{4}{c}{\textbf{CoT}} & \multicolumn{4}{c}{\textbf{Few-shot}} \\ 

 \cline{3-18}
  % \rowcolor{gray!30}
 &  & \textbf{ECE} & \textbf{t-ECE} & \textbf{Brier} & \textbf{AUC} 
    & \textbf{ECE} & \textbf{t-ECE} & \textbf{Brier} & \textbf{AUC} 
    & \textbf{ECE} & \textbf{t-ECE} & \textbf{Brier} & \textbf{AUC}  
    & \textbf{ECE} & \textbf{t-ECE} & \textbf{Brier} & \textbf{AUC} \\ 

\hline
 \input{latex/tables/text/deberta_nq_large}

\end{tabular}
\caption{Test performance of our methods (Calib-*) and baseline methods on NQ dataset using four different prompts (Verb., Zero-shot, CoT, Few-shot). Only Verb. prompt asks the LLM to provide a probability for a given answer and thus have the results for Verblized Prob. performance. We color the text with a scale normalized by the values gap in each column,  where red indicates better and green presents worse performance. The results of the other three datasets are shown in Appendix.}\label{tb:nq_large}
\end{table*}

==> tables/large_model_results.tex <==
% \begin{table*}[h!]
% \centering
% \scriptsize
% \begin{tabular}{c|c|l@{\hspace{0.25cm}}l@{\hspace{0.25cm}}l@{\hspace{0.25cm}}l@{\hspace{0.25cm}}|l@{\hspace{0.25cm}}l@{\hspace{0.25cm}}l@{\hspace{0.25cm}}l@{\hspace{0.25cm}}|l@{\hspace{0.25cm}}l@{\hspace{0.25cm}}l@{\hspace{0.25cm}}l@{\hspace{0.25cm}}|l@{\hspace{0.25cm}}l@{\hspace{0.25cm}}l@{\hspace{0.25cm}}l@{\hspace{0.25cm}}}
% \hline
%  & & \multicolumn{4}{c}{Verb.} & \multicolumn{4}{c}{Zero-shot}&  \multicolumn{4}{c}{CoT}& \multicolumn{4}{c}{Few-shot} \\ \hline
%  {model} & {method} &{ECE} & {t-ECE} & {Brier} & {AUC} & {ECE} & {t-ECE} & {Brier} & {AUC} & {ECE} & {t-ECE} & {Brier} & {AUC}  & {ECE} & {t-ECE} & {Brier} & {AUC} \\ \hline
 
% \input{latex/tables/text/large_model_results_text}

% \end{tabular}
% \caption{Sample Table from CSV Data}
% \end{table*}

==> tables/model_performance.tex <==
\begin{table*}[h!]
\centering
\scriptsize
\begin{tabular}{c|l@{\hspace{0.25cm}}l@{\hspace{0.25cm}}l@{\hspace{0.25cm}}l@{\hspace{0.25cm}}|l@{\hspace{0.25cm}}l@{\hspace{0.25cm}}l@{\hspace{0.25cm}}l@{\hspace{0.25cm}}|l@{\hspace{0.25cm}}l@{\hspace{0.25cm}}l@{\hspace{0.25cm}}l@{\hspace{0.25cm}}|l@{\hspace{0.25cm}}l@{\hspace{0.25cm}}l@{\hspace{0.25cm}}l@{\hspace{0.25cm}}}
\hline
 {prompt} &{model} & {success} & {acc} & {success} & {acc}  & {success} & {acc}  & {success} & {acc}   \\ \hline
 0.325 &0.325 & 0.325&0.325 & En&0.325 & 0.325&0.325 & 0.325&0.325 \\ \hline
 
 0.325 &0.325 & 0.325&0.325 & En&0.325 & 0.325&0.325 & 0.325&0.325\\ \hline
 
 0.325 &0.325 & 0.325&0.325 & En&0.325 & 0.325&0.325 & 0.325&0.325 \\ \hline
 
 0.325 &0.325 & 0.325&0.325 & En&0.325 & 0.325&0.325 & 0.325&0.325 \\ \hline
\end{tabular}
\caption{Sample Table from CSV Data}
\end{table*}

==> tables/text/deberta_nq_large.tex <==
\multirow{8}{*}{\rotatebox{90}{Gemma2-27b}} & LLM Prob. & \cellcolor[HTML]{FCE2A2}0.445 & \cellcolor[HTML]{FEF6BB}0.249 & \cellcolor[HTML]{FBDA98}0.417 & \cellcolor[HTML]{EC7014}0.704 & \cellcolor[HTML]{FEF6BB}0.447 & \cellcolor[HTML]{FEF6BB}0.255 & \cellcolor[HTML]{FEF6BB}0.419 & \cellcolor[HTML]{EC7014}0.713 & \cellcolor[HTML]{FEF6BB}0.395 & \cellcolor[HTML]{FEF6BB}0.268 & \cellcolor[HTML]{FEF6BB}0.392 & \cellcolor[HTML]{FFF7BC}0.671 & \cellcolor[HTML]{FEF6BB}0.235 & \cellcolor[HTML]{FEF6BB}0.184 & \cellcolor[HTML]{FEF6BB}0.308 & \cellcolor[HTML]{FFF7BC}0.584 \\
  & LLM Prob.+PS & \cellcolor[HTML]{F5B166}0.282 & \cellcolor[HTML]{EC7014}0.052 & \cellcolor[HTML]{F19A48}0.293 & \cellcolor[HTML]{EE832C}0.690 & \cellcolor[HTML]{F6B96F}0.276 & \cellcolor[HTML]{EC7014}0.064 & \cellcolor[HTML]{F29D4C}0.288 & \cellcolor[HTML]{EC7014}0.713 & \cellcolor[HTML]{F4AD60}0.226 & \cellcolor[HTML]{EC7014}0.059 & \cellcolor[HTML]{F29E4D}0.283 & \cellcolor[HTML]{FEF2B6}0.672 & \cellcolor[HTML]{F19644}0.133 & \cellcolor[HTML]{EC7014}0.011 & \cellcolor[HTML]{F5B267}0.264 & \cellcolor[HTML]{FFF7BC}0.584 \\
  & Verblized Prob. & \cellcolor[HTML]{FEF6BB}0.512 & \cellcolor[HTML]{F9CC87}0.187 & \cellcolor[HTML]{FEF6BB}0.471 & \cellcolor[HTML]{EF8A34}0.685 & nan00 & nan00 & nan00 & nan00 & nan00 & nan00 & nan00 & nan00 & nan00 & nan00 & nan00 & nan00 \\
  & APRICOT & \cellcolor[HTML]{EE7E26}0.111 & \cellcolor[HTML]{F08C37}0.094 & \cellcolor[HTML]{ED781E}0.228 & \cellcolor[HTML]{FFF7BC}0.607 & \cellcolor[HTML]{ED7D24}0.110 & \cellcolor[HTML]{F19440}0.115 & \cellcolor[HTML]{EC761C}0.232 & \cellcolor[HTML]{FFF7BC}0.627 & \cellcolor[HTML]{EC7015}0.087 & \cellcolor[HTML]{ED7B22}0.077 & \cellcolor[HTML]{EC7014}0.226 & \cellcolor[HTML]{FAD896}0.678 & \cellcolor[HTML]{EC7014}0.092 & \cellcolor[HTML]{F4AD60}0.090 & \cellcolor[HTML]{EF852F}0.235 & \cellcolor[HTML]{F29F4F}0.678 \\
 [0.2em] \cline{2-18} 
   & (BCE)Calib-1 & \cellcolor[HTML]{EC7014}0.064 & \cellcolor[HTML]{EC761C}0.062 & \cellcolor[HTML]{EC7014}0.213 & \cellcolor[HTML]{F6BC73}0.649 & \cellcolor[HTML]{EC7014}0.073 & \cellcolor[HTML]{ED791F}0.077 & \cellcolor[HTML]{EC7014}0.222 & \cellcolor[HTML]{FBE1A0}0.641 & \cellcolor[HTML]{ED791F}0.107 & \cellcolor[HTML]{EE8028}0.085 & \cellcolor[HTML]{EC761C}0.234 & \cellcolor[HTML]{FEF2B6}0.672 & \cellcolor[HTML]{F5B266}0.162 & \cellcolor[HTML]{FCE3A3}0.159 & \cellcolor[HTML]{F08F3A}0.241 & \cellcolor[HTML]{ED791F}0.719 \\
  & (BCE)Calib-n & \cellcolor[HTML]{EF8630}0.138 & \cellcolor[HTML]{F4AA5D}0.138 & \cellcolor[HTML]{ED781F}0.229 & \cellcolor[HTML]{F29D4D}0.671 & \cellcolor[HTML]{F0923E}0.168 & \cellcolor[HTML]{F6B86D}0.166 & \cellcolor[HTML]{EE7F27}0.245 & \cellcolor[HTML]{F7C179}0.661 & \cellcolor[HTML]{EF8832}0.141 & \cellcolor[HTML]{F3A455}0.140 & \cellcolor[HTML]{ED7920}0.238 & \cellcolor[HTML]{EE8129}0.698 & \cellcolor[HTML]{F08D38}0.123 & \cellcolor[HTML]{F6BC73}0.109 & \cellcolor[HTML]{ED771D}0.226 & \cellcolor[HTML]{EC751A}0.723 \\
  & (FL)Calib-1 & \cellcolor[HTML]{EC7014}0.062 & \cellcolor[HTML]{ED7B22}0.069 & \cellcolor[HTML]{EC7014}0.212 & \cellcolor[HTML]{F5B66C}0.653 & \cellcolor[HTML]{EC751A}0.088 & \cellcolor[HTML]{EF852F}0.095 & \cellcolor[HTML]{EC7014}0.222 & \cellcolor[HTML]{FBDC9A}0.644 & \cellcolor[HTML]{EC7014}0.085 & \cellcolor[HTML]{EE822A}0.087 & \cellcolor[HTML]{EC7318}0.230 & \cellcolor[HTML]{FCE5A6}0.675 & \cellcolor[HTML]{EE822B}0.112 & \cellcolor[HTML]{F7C57D}0.120 & \cellcolor[HTML]{ED771D}0.226 & \cellcolor[HTML]{EC7014}0.729 \\
  & (FL)Calib-n & \cellcolor[HTML]{EF8832}0.145 & \cellcolor[HTML]{F4AF62}0.144 & \cellcolor[HTML]{ED7920}0.231 & \cellcolor[HTML]{F29D4D}0.671 & \cellcolor[HTML]{F08F3B}0.160 & \cellcolor[HTML]{F5B368}0.160 & \cellcolor[HTML]{EE7E25}0.243 & \cellcolor[HTML]{F7C077}0.662 & \cellcolor[HTML]{EE8028}0.122 & \cellcolor[HTML]{F29B49}0.126 & \cellcolor[HTML]{EC751B}0.233 & \cellcolor[HTML]{EC7014}0.702 & \cellcolor[HTML]{EC751B}0.098 & \cellcolor[HTML]{F4AC5E}0.088 & \cellcolor[HTML]{EC7014}0.221 & \cellcolor[HTML]{EC7318}0.725 \\
\hline \hline 
\multirow{8}{*}{\rotatebox{90}{Llama3-70b}} & LLM Prob. & \cellcolor[HTML]{FEF6BB}0.445 & \cellcolor[HTML]{FEF6BB}0.302 & \cellcolor[HTML]{FEF6BB}0.430 & \cellcolor[HTML]{EC7014}0.712 & \cellcolor[HTML]{FEF6BB}0.458 & \cellcolor[HTML]{FEF6BB}0.259 & \cellcolor[HTML]{FEF6BB}0.426 & \cellcolor[HTML]{EC7014}0.747 & \cellcolor[HTML]{FEF6BB}0.412 & \cellcolor[HTML]{FEF6BB}0.251 & \cellcolor[HTML]{FEF6BB}0.416 & \cellcolor[HTML]{FFF7BC}0.612 & \cellcolor[HTML]{FEF6BB}0.336 & \cellcolor[HTML]{FBE09F}0.117 & \cellcolor[HTML]{FEF6BB}0.364 & \cellcolor[HTML]{FFF7BC}0.532 \\
  & LLM Prob.+PS & \cellcolor[HTML]{F9D18D}0.355 & \cellcolor[HTML]{EE812A}0.113 & \cellcolor[HTML]{F7BE75}0.350 & \cellcolor[HTML]{ED7A21}0.703 & \cellcolor[HTML]{F5B367}0.266 & \cellcolor[HTML]{F19948}0.132 & \cellcolor[HTML]{F29A49}0.291 & \cellcolor[HTML]{EC7014}0.747 & \cellcolor[HTML]{F3A152}0.224 & \cellcolor[HTML]{EC7014}0.023 & \cellcolor[HTML]{F0933F}0.289 & \cellcolor[HTML]{FFF7BC}0.612 & \cellcolor[HTML]{F7BE76}0.224 & \cellcolor[HTML]{EC7014}0.009 & \cellcolor[HTML]{F6B96F}0.298 & \cellcolor[HTML]{FFF7BC}0.532 \\
  & Verblized Prob. & \cellcolor[HTML]{FCE6A7}0.406 & \cellcolor[HTML]{EC7014}0.084 & \cellcolor[HTML]{FAD390}0.380 & \cellcolor[HTML]{EE8028}0.698 & nan00 & nan00 & nan00 & nan00 & nan00 & nan00 & nan00 & nan00 & nan00 & nan00 & nan00 & nan00 \\
  & APRICOT & \cellcolor[HTML]{EC761B}0.137 & \cellcolor[HTML]{F08C37}0.130 & \cellcolor[HTML]{ED7B22}0.255 & \cellcolor[HTML]{FFF7BC}0.596 & \cellcolor[HTML]{ED7C23}0.111 & \cellcolor[HTML]{F08E39}0.116 & \cellcolor[HTML]{ED771D}0.239 & \cellcolor[HTML]{FEF3B7}0.635 & \cellcolor[HTML]{EC7014}0.114 & \cellcolor[HTML]{F3A759}0.117 & \cellcolor[HTML]{EC7014}0.244 & \cellcolor[HTML]{F29F4F}0.656 & \cellcolor[HTML]{EE832C}0.106 & \cellcolor[HTML]{F4AD60}0.068 & \cellcolor[HTML]{EE7F27}0.236 & \cellcolor[HTML]{EF8C37}0.683 \\
 [0.2em] \cline{2-18} 
   & (BCE)Calib-1 & \cellcolor[HTML]{EC7014}0.122 & \cellcolor[HTML]{EF8B36}0.129 & \cellcolor[HTML]{EC7014}0.239 & \cellcolor[HTML]{F9D28F}0.627 & \cellcolor[HTML]{EC7014}0.076 & \cellcolor[HTML]{EC7014}0.075 & \cellcolor[HTML]{EC7014}0.228 & \cellcolor[HTML]{FFF7BC}0.632 & \cellcolor[HTML]{EE832B}0.156 & \cellcolor[HTML]{F7C179}0.161 & \cellcolor[HTML]{EC761B}0.252 & \cellcolor[HTML]{EC7318}0.678 & \cellcolor[HTML]{F19542}0.141 & \cellcolor[HTML]{FEF6BB}0.139 & \cellcolor[HTML]{EE7F27}0.236 & \cellcolor[HTML]{EC761B}0.714 \\
  & (BCE)Calib-n & \cellcolor[HTML]{ED7A20}0.146 & \cellcolor[HTML]{F29C4B}0.156 & \cellcolor[HTML]{EC7216}0.242 & \cellcolor[HTML]{F4AC5F}0.660 & \cellcolor[HTML]{F0903C}0.169 & \cellcolor[HTML]{F4AC5E}0.157 & \cellcolor[HTML]{ED7C24}0.247 & \cellcolor[HTML]{F8C983}0.671 & \cellcolor[HTML]{EF8730}0.165 & \cellcolor[HTML]{F7C47D}0.166 & \cellcolor[HTML]{EC771C}0.253 & \cellcolor[HTML]{ED771D}0.676 & \cellcolor[HTML]{EF8731}0.114 & \cellcolor[HTML]{F8C67F}0.092 & \cellcolor[HTML]{EC7318}0.223 & \cellcolor[HTML]{EC7014}0.723 \\
  & (FL)Calib-1 & \cellcolor[HTML]{EE7F26}0.158 & \cellcolor[HTML]{F29B4A}0.155 & \cellcolor[HTML]{ED771D}0.250 & \cellcolor[HTML]{F9D08C}0.629 & \cellcolor[HTML]{EC741A}0.090 & \cellcolor[HTML]{ED7D24}0.093 & \cellcolor[HTML]{EC7014}0.229 & \cellcolor[HTML]{FDEDB0}0.640 & \cellcolor[HTML]{EE8028}0.151 & \cellcolor[HTML]{F6BA70}0.149 & \cellcolor[HTML]{EC7216}0.247 & \cellcolor[HTML]{EC7014}0.680 & \cellcolor[HTML]{EC7014}0.066 & \cellcolor[HTML]{F29C4B}0.052 & \cellcolor[HTML]{EC7014}0.219 & \cellcolor[HTML]{EC7318}0.718 \\
  & (FL)Calib-n & \cellcolor[HTML]{ED7A20}0.146 & \cellcolor[HTML]{F19A48}0.152 & \cellcolor[HTML]{EC7014}0.240 & \cellcolor[HTML]{F29F4F}0.671 & \cellcolor[HTML]{EF8C37}0.156 & \cellcolor[HTML]{F3A759}0.151 & \cellcolor[HTML]{ED781F}0.241 & \cellcolor[HTML]{F7C47D}0.675 & \cellcolor[HTML]{EE7E26}0.146 & \cellcolor[HTML]{F6BC73}0.152 & \cellcolor[HTML]{EC7317}0.248 & \cellcolor[HTML]{EC7318}0.678 & \cellcolor[HTML]{EE822B}0.103 & \cellcolor[HTML]{F6BC73}0.083 & \cellcolor[HTML]{EC7217}0.222 & \cellcolor[HTML]{EC7014}0.723 \\
\hline \hline 
\multirow{8}{*}{\rotatebox{90}{Llama3.1-70b}} & LLM Prob. & \cellcolor[HTML]{F7C27A}0.301 & \cellcolor[HTML]{FEF6BB}0.231 & \cellcolor[HTML]{F6BB71}0.326 & \cellcolor[HTML]{ED7A21}0.704 & \cellcolor[HTML]{FEF6BB}0.308 & \cellcolor[HTML]{FEF6BB}0.237 & \cellcolor[HTML]{FEF6BB}0.326 & \cellcolor[HTML]{EC7014}0.722 & \cellcolor[HTML]{FEF6BB}0.274 & \cellcolor[HTML]{FEF6BB}0.221 & \cellcolor[HTML]{FEF6BB}0.330 & \cellcolor[HTML]{FFF7BC}0.619 & \cellcolor[HTML]{FEF6BB}0.172 & \cellcolor[HTML]{F5B469}0.098 & \cellcolor[HTML]{FEF6BB}0.266 & \cellcolor[HTML]{FFF7BC}0.640 \\
  & LLM Prob.+PS & \cellcolor[HTML]{F5B063}0.254 & \cellcolor[HTML]{EE832C}0.116 & \cellcolor[HTML]{F3A252}0.293 & \cellcolor[HTML]{F08F3B}0.690 & \cellcolor[HTML]{F9CD88}0.236 & \cellcolor[HTML]{EC7014}0.066 & \cellcolor[HTML]{F5B468}0.279 & \cellcolor[HTML]{EC7014}0.722 & \cellcolor[HTML]{F7BF76}0.195 & \cellcolor[HTML]{EC7014}0.023 & \cellcolor[HTML]{F5B063}0.275 & \cellcolor[HTML]{FFF7BC}0.619 & \cellcolor[HTML]{F5B66C}0.135 & \cellcolor[HTML]{EC7014}0.064 & \cellcolor[HTML]{FCE2A2}0.258 & \cellcolor[HTML]{FFF7BC}0.640 \\
  & Verblized Prob. & \cellcolor[HTML]{FEF6BB}0.435 & \cellcolor[HTML]{EF8934}0.122 & \cellcolor[HTML]{FEF6BB}0.405 & \cellcolor[HTML]{EC7014}0.711 & nan00 & nan00 & nan00 & nan00 & nan00 & nan00 & nan00 & nan00 & nan00 & nan00 & nan00 & nan00 \\
  & APRICOT & \cellcolor[HTML]{ED7B22}0.120 & \cellcolor[HTML]{EE822B}0.115 & \cellcolor[HTML]{EE8028}0.248 & \cellcolor[HTML]{FFF7BC}0.621 & \cellcolor[HTML]{EC7217}0.080 & \cellcolor[HTML]{ED791F}0.078 & \cellcolor[HTML]{ED7B22}0.239 & \cellcolor[HTML]{FFF7BC}0.635 & \cellcolor[HTML]{EC7014}0.083 & \cellcolor[HTML]{F19644}0.080 & \cellcolor[HTML]{EC761B}0.230 & \cellcolor[HTML]{F3A556}0.688 & \cellcolor[HTML]{EC751A}0.097 & \cellcolor[HTML]{EF862F}0.075 & \cellcolor[HTML]{F3A354}0.234 & \cellcolor[HTML]{F6B86D}0.687 \\
 [0.2em] \cline{2-18} 
   & (BCE)Calib-1 & \cellcolor[HTML]{EC7014}0.090 & \cellcolor[HTML]{EC741A}0.101 & \cellcolor[HTML]{EC7014}0.226 & \cellcolor[HTML]{F29D4C}0.681 & \cellcolor[HTML]{EC7216}0.079 & \cellcolor[HTML]{EF8832}0.097 & \cellcolor[HTML]{EC7217}0.233 & \cellcolor[HTML]{FBDE9D}0.651 & \cellcolor[HTML]{F4AC5F}0.169 & \cellcolor[HTML]{F9CD88}0.160 & \cellcolor[HTML]{EE812A}0.239 & \cellcolor[HTML]{EC7115}0.732 & \cellcolor[HTML]{F3A758}0.126 & \cellcolor[HTML]{FEF6BB}0.131 & \cellcolor[HTML]{F08C37}0.225 & \cellcolor[HTML]{EC751A}0.737 \\
  & (BCE)Calib-n & \cellcolor[HTML]{EE7E26}0.127 & \cellcolor[HTML]{EF8A35}0.123 & \cellcolor[HTML]{EC761C}0.235 & \cellcolor[HTML]{F3A455}0.676 & \cellcolor[HTML]{F3A759}0.171 & \cellcolor[HTML]{F5B76C}0.156 & \cellcolor[HTML]{F19441}0.257 & \cellcolor[HTML]{FAD997}0.654 & \cellcolor[HTML]{F0913D}0.130 & \cellcolor[HTML]{F5B267}0.121 & \cellcolor[HTML]{EC7318}0.228 & \cellcolor[HTML]{EC751B}0.728 & \cellcolor[HTML]{EC761C}0.098 & \cellcolor[HTML]{F3A85A}0.092 & \cellcolor[HTML]{EC7217}0.215 & \cellcolor[HTML]{ED791F}0.734 \\
  & (FL)Calib-1 & \cellcolor[HTML]{EC7217}0.097 & \cellcolor[HTML]{EC7014}0.096 & \cellcolor[HTML]{EC7115}0.228 & \cellcolor[HTML]{F29E4D}0.680 & \cellcolor[HTML]{EC7014}0.075 & \cellcolor[HTML]{EE832C}0.091 & \cellcolor[HTML]{EC7014}0.231 & \cellcolor[HTML]{FAD693}0.656 & \cellcolor[HTML]{F19644}0.138 & \cellcolor[HTML]{F6BA70}0.132 & \cellcolor[HTML]{EC751A}0.229 & \cellcolor[HTML]{EC7014}0.733 & \cellcolor[HTML]{ED7D25}0.102 & \cellcolor[HTML]{F9CC87}0.110 & \cellcolor[HTML]{ED771D}0.217 & \cellcolor[HTML]{EC7014}0.741 \\
  & (FL)Calib-n & \cellcolor[HTML]{EE8129}0.134 & \cellcolor[HTML]{F0923F}0.131 & \cellcolor[HTML]{ED771D}0.236 & \cellcolor[HTML]{F3A657}0.675 & \cellcolor[HTML]{F29D4C}0.153 & \cellcolor[HTML]{F4AC5F}0.143 & \cellcolor[HTML]{EF8A35}0.250 & \cellcolor[HTML]{F9D08B}0.660 & \cellcolor[HTML]{EF8933}0.119 & \cellcolor[HTML]{F3A657}0.103 & \cellcolor[HTML]{EC7014}0.225 & \cellcolor[HTML]{ED771C}0.727 & \cellcolor[HTML]{EC7014}0.094 & \cellcolor[HTML]{F19A48}0.085 & \cellcolor[HTML]{EC7014}0.214 & \cellcolor[HTML]{ED7A21}0.733 \\
\hline \hline 
\multirow{8}{*}{\rotatebox{90}{Qwen2-72b}} & LLM Prob. & \cellcolor[HTML]{FEF6BB}0.470 & \cellcolor[HTML]{FEF6BB}0.321 & \cellcolor[HTML]{FEF6BB}0.455 & \cellcolor[HTML]{F3A657}0.692 & \cellcolor[HTML]{FEF6BB}0.483 & \cellcolor[HTML]{FEF6BB}0.280 & \cellcolor[HTML]{FEF6BB}0.450 & \cellcolor[HTML]{EC7014}0.734 & \cellcolor[HTML]{FEF6BB}0.380 & \cellcolor[HTML]{FEF6BB}0.276 & \cellcolor[HTML]{FEF6BB}0.393 & \cellcolor[HTML]{FFF7BC}0.620 & \cellcolor[HTML]{FEF6BB}0.220 & \cellcolor[HTML]{F19441}0.092 & \cellcolor[HTML]{FEF4B9}0.280 & \cellcolor[HTML]{FFF7BC}0.645 \\
  & LLM Prob.+PS & \cellcolor[HTML]{F4AE61}0.259 & \cellcolor[HTML]{F08D38}0.120 & \cellcolor[HTML]{F19441}0.289 & \cellcolor[HTML]{EC7014}0.745 & \cellcolor[HTML]{F5B165}0.270 & \cellcolor[HTML]{EC7014}0.057 & \cellcolor[HTML]{F29B4A}0.292 & \cellcolor[HTML]{EC7014}0.734 & \cellcolor[HTML]{F29C4B}0.202 & \cellcolor[HTML]{EC7014}0.021 & \cellcolor[HTML]{F0913D}0.282 & \cellcolor[HTML]{FFF7BC}0.620 & \cellcolor[HTML]{FCE6A7}0.203 & \cellcolor[HTML]{EE822A}0.085 & \cellcolor[HTML]{FEF6BB}0.281 & \cellcolor[HTML]{FFF7BC}0.645 \\
  & Verblized Prob. & \cellcolor[HTML]{FDEAAC}0.433 & \cellcolor[HTML]{EC7014}0.065 & \cellcolor[HTML]{FAD896}0.404 & \cellcolor[HTML]{ED7B22}0.734 & nan00 & nan00 & nan00 & nan00 & nan00 & nan00 & nan00 & nan00 & nan00 & nan00 & nan00 & nan00 \\
  & APRICOT & \cellcolor[HTML]{ED7C23}0.114 & \cellcolor[HTML]{EF8933}0.113 & \cellcolor[HTML]{ED781E}0.241 & \cellcolor[HTML]{FFF7BC}0.614 & \cellcolor[HTML]{ED781E}0.096 & \cellcolor[HTML]{EE8029}0.085 & \cellcolor[HTML]{EC751B}0.227 & \cellcolor[HTML]{FFF7BC}0.647 & \cellcolor[HTML]{EC7014}0.113 & \cellcolor[HTML]{F2A04F}0.112 & \cellcolor[HTML]{EC7015}0.247 & \cellcolor[HTML]{F8C67F}0.641 & \cellcolor[HTML]{EC751B}0.086 & \cellcolor[HTML]{EC7014}0.078 & \cellcolor[HTML]{F08E3A}0.230 & \cellcolor[HTML]{F4AE61}0.694 \\
 [0.2em] \cline{2-18} 
   & (BCE)Calib-1 & \cellcolor[HTML]{EC7014}0.079 & \cellcolor[HTML]{ED7A21}0.085 & \cellcolor[HTML]{EC7014}0.227 & \cellcolor[HTML]{F8C882}0.659 & \cellcolor[HTML]{EC7014}0.071 & \cellcolor[HTML]{EE822B}0.088 & \cellcolor[HTML]{EC7014}0.218 & \cellcolor[HTML]{F9D18D}0.671 & \cellcolor[HTML]{F08F3B}0.176 & \cellcolor[HTML]{F8C67F}0.184 & \cellcolor[HTML]{ED7C23}0.260 & \cellcolor[HTML]{EF8B36}0.666 & \cellcolor[HTML]{F29E4D}0.128 & \cellcolor[HTML]{FEF6BB}0.130 & \cellcolor[HTML]{F08E3A}0.230 & \cellcolor[HTML]{EF862F}0.721 \\
  & (BCE)Calib-n & \cellcolor[HTML]{EE822A}0.132 & \cellcolor[HTML]{F0913D}0.128 & \cellcolor[HTML]{EC7419}0.234 & \cellcolor[HTML]{F6B86D}0.675 & \cellcolor[HTML]{F08E3A}0.163 & \cellcolor[HTML]{F3A85A}0.150 & \cellcolor[HTML]{ED7D25}0.241 & \cellcolor[HTML]{F8C57E}0.679 & \cellcolor[HTML]{EF8B35}0.167 & \cellcolor[HTML]{F6B96F}0.160 & \cellcolor[HTML]{ED7A20}0.257 & \cellcolor[HTML]{EC761C}0.675 & \cellcolor[HTML]{EF8730}0.104 & \cellcolor[HTML]{F4A95B}0.100 & \cellcolor[HTML]{ED7C23}0.221 & \cellcolor[HTML]{ED781F}0.730 \\
  & (FL)Calib-1 & \cellcolor[HTML]{ED7D25}0.119 & \cellcolor[HTML]{F08C37}0.119 & \cellcolor[HTML]{EC7216}0.231 & \cellcolor[HTML]{F7BE75}0.669 & \cellcolor[HTML]{EC7014}0.069 & \cellcolor[HTML]{EE8029}0.085 & \cellcolor[HTML]{EC7014}0.217 & \cellcolor[HTML]{F8C882}0.677 & \cellcolor[HTML]{ED7B21}0.135 & \cellcolor[HTML]{F5B368}0.149 & \cellcolor[HTML]{EC7014}0.246 & \cellcolor[HTML]{EE842E}0.669 & \cellcolor[HTML]{EF8730}0.104 & \cellcolor[HTML]{F7C078}0.109 & \cellcolor[HTML]{EE822A}0.224 & \cellcolor[HTML]{EF862F}0.721 \\
  & (FL)Calib-n & \cellcolor[HTML]{EE842D}0.139 & \cellcolor[HTML]{F19745}0.140 & \cellcolor[HTML]{EC7419}0.235 & \cellcolor[HTML]{F6B86D}0.675 & \cellcolor[HTML]{EF8731}0.142 & \cellcolor[HTML]{F3A454}0.143 & \cellcolor[HTML]{ED7B21}0.236 & \cellcolor[HTML]{F7BF76}0.683 & \cellcolor[HTML]{EF862F}0.157 & \cellcolor[HTML]{F5B165}0.144 & \cellcolor[HTML]{EC7419}0.251 & \cellcolor[HTML]{EC7014}0.678 & \cellcolor[HTML]{EC7014}0.080 & \cellcolor[HTML]{EC7217}0.079 & \cellcolor[HTML]{EC7014}0.215 & \cellcolor[HTML]{EC7014}0.736 \\
\hline \hline 
\multirow{8}{*}{\rotatebox{90}{Mixtral-8x7b}} & LLM Prob. & \cellcolor[HTML]{FEF6BB}0.513 & \cellcolor[HTML]{FEF6BB}0.269 & \cellcolor[HTML]{FEF6BB}0.479 & \cellcolor[HTML]{EC7014}0.703 & \cellcolor[HTML]{FEF6BB}0.412 & \cellcolor[HTML]{FEF6BB}0.155 & \cellcolor[HTML]{FEF6BB}0.401 & \cellcolor[HTML]{FFF7BC}0.637 & \cellcolor[HTML]{FEF6BB}0.452 & \cellcolor[HTML]{FEF6BB}0.270 & \cellcolor[HTML]{FEF6BB}0.447 & \cellcolor[HTML]{FCE3A4}0.627 & \cellcolor[HTML]{FEF6BB}0.369 & \cellcolor[HTML]{FADA98}0.075 & \cellcolor[HTML]{FEF6BB}0.380 & \cellcolor[HTML]{FFF7BC}0.574 \\
  & LLM Prob.+PS & \cellcolor[HTML]{F4A95C}0.264 & \cellcolor[HTML]{EC7014}0.015 & \cellcolor[HTML]{F0923E}0.292 & \cellcolor[HTML]{F5B267}0.653 & \cellcolor[HTML]{F4AE61}0.233 & \cellcolor[HTML]{EC7014}0.066 & \cellcolor[HTML]{F2A050}0.290 & \cellcolor[HTML]{FFF7BC}0.637 & \cellcolor[HTML]{F3A454}0.245 & \cellcolor[HTML]{EC7014}0.013 & \cellcolor[HTML]{F19745}0.305 & \cellcolor[HTML]{FCE3A4}0.627 & \cellcolor[HTML]{F08D39}0.141 & \cellcolor[HTML]{EC7014}0.001 & \cellcolor[HTML]{F19643}0.267 & \cellcolor[HTML]{FFF7BC}0.574 \\
  & Verblized Prob. & \cellcolor[HTML]{FDEAAC}0.472 & \cellcolor[HTML]{F7C078}0.167 & \cellcolor[HTML]{FCE5A6}0.447 & \cellcolor[HTML]{F5B063}0.655 & nan00 & nan00 & nan00 & nan00 & nan00 & nan00 & nan00 & nan00 & nan00 & nan00 & nan00 & nan00 \\
  & APRICOT & \cellcolor[HTML]{EE7E26}0.124 & \cellcolor[HTML]{F3A759}0.120 & \cellcolor[HTML]{ED7920}0.247 & \cellcolor[HTML]{FFF7BC}0.602 & \cellcolor[HTML]{EC751A}0.092 & \cellcolor[HTML]{F0913D}0.088 & \cellcolor[HTML]{ED791F}0.239 & \cellcolor[HTML]{FAD997}0.646 & \cellcolor[HTML]{EC7014}0.115 & \cellcolor[HTML]{F3A455}0.113 & \cellcolor[HTML]{EC7419}0.252 & \cellcolor[HTML]{FFF7BC}0.620 & \cellcolor[HTML]{F19744}0.161 & \cellcolor[HTML]{F9D38F}0.070 & \cellcolor[HTML]{F0933F}0.263 & \cellcolor[HTML]{F5B66B}0.640 \\
 [0.2em] \cline{2-18} 
   & (BCE)Calib-1 & \cellcolor[HTML]{EC7116}0.083 & \cellcolor[HTML]{F19948}0.094 & \cellcolor[HTML]{EC7014}0.230 & \cellcolor[HTML]{FAD997}0.624 & \cellcolor[HTML]{ED781E}0.099 & \cellcolor[HTML]{F2A050}0.098 & \cellcolor[HTML]{ED781E}0.238 & \cellcolor[HTML]{F4AB5D}0.660 & \cellcolor[HTML]{EE842C}0.165 & \cellcolor[HTML]{F7C37B}0.172 & \cellcolor[HTML]{ED7A21}0.262 & \cellcolor[HTML]{F0913D}0.657 & \cellcolor[HTML]{F0903C}0.147 & \cellcolor[HTML]{FEF6BB}0.095 & \cellcolor[HTML]{EF8832}0.251 & \cellcolor[HTML]{ED7D25}0.698 \\
  & (BCE)Calib-n & \cellcolor[HTML]{EE822B}0.138 & \cellcolor[HTML]{F5B165}0.138 & \cellcolor[HTML]{EC7419}0.237 & \cellcolor[HTML]{F5B267}0.653 & \cellcolor[HTML]{EC751A}0.092 & \cellcolor[HTML]{F08C37}0.085 & \cellcolor[HTML]{EC7216}0.230 & \cellcolor[HTML]{ED7920}0.675 & \cellcolor[HTML]{ED791F}0.139 & \cellcolor[HTML]{F5B56A}0.146 & \cellcolor[HTML]{EC7419}0.253 & \cellcolor[HTML]{ED7D25}0.664 & \cellcolor[HTML]{ED771D}0.092 & \cellcolor[HTML]{FBE1A1}0.080 & \cellcolor[HTML]{EC7116}0.224 & \cellcolor[HTML]{EC7015}0.711 \\
  & (FL)Calib-1 & \cellcolor[HTML]{EC7014}0.077 & \cellcolor[HTML]{F19745}0.090 & \cellcolor[HTML]{EC7014}0.229 & \cellcolor[HTML]{FAD997}0.624 & \cellcolor[HTML]{ED7920}0.103 & \cellcolor[HTML]{F5B267}0.110 & \cellcolor[HTML]{EC761B}0.235 & \cellcolor[HTML]{F29E4D}0.664 & \cellcolor[HTML]{EE8028}0.157 & \cellcolor[HTML]{F6BC72}0.158 & \cellcolor[HTML]{EC761C}0.256 & \cellcolor[HTML]{ED781E}0.666 & \cellcolor[HTML]{EE832C}0.118 & \cellcolor[HTML]{F8C781}0.062 & \cellcolor[HTML]{EE7E26}0.239 & \cellcolor[HTML]{EE7E26}0.697 \\
  & (FL)Calib-n & \cellcolor[HTML]{EE8129}0.132 & \cellcolor[HTML]{F4AD60}0.130 & \cellcolor[HTML]{EC7419}0.237 & \cellcolor[HTML]{F3A859}0.661 & \cellcolor[HTML]{EC7014}0.079 & \cellcolor[HTML]{EF8630}0.081 & \cellcolor[HTML]{EC7014}0.227 & \cellcolor[HTML]{EC7014}0.678 & \cellcolor[HTML]{EC761C}0.132 & \cellcolor[HTML]{F4AB5E}0.127 & \cellcolor[HTML]{EC7014}0.246 & \cellcolor[HTML]{EC7014}0.669 & \cellcolor[HTML]{EC7014}0.076 & \cellcolor[HTML]{FAD491}0.071 & \cellcolor[HTML]{EC7014}0.222 & \cellcolor[HTML]{EC7014}0.712 \\
\hline \hline 


==> tables/text/large_model_results_text.tex <==
gemma2-27b & LLM Prob. & {\color[HTML]{59B900} 0.339} & {\color[HTML]{32E000} 0.235} & {\color[HTML]{6DA500} 0.336} & {\color[HTML]{E03200} 0.721} & {\color[HTML]{32E000} 0.354} & {\color[HTML]{32E000} 0.23} & {\color[HTML]{32E000} 0.343} & {\color[HTML]{E03200} 0.721} & {\color[HTML]{32E000} 0.293} & {\color[HTML]{32E000} 0.226} & {\color[HTML]{32E000} 0.321} & {\color[HTML]{DF3300} 0.637} & {\color[HTML]{35DD00} 0.152} & {\color[HTML]{35DD00} 0.152} & {\color[HTML]{32E000} 0.233} & {\color[HTML]{D63C00} 0.566} \\
gemma2-27b & LLM Prob + PS & {\color[HTML]{A86A00} 0.186} & {\color[HTML]{E13200} 0.052} & {\color[HTML]{B95900} 0.26} & {\color[HTML]{A66C00} 0.685} & {\color[HTML]{48CA00} 0.18} & {\color[HTML]{47CB00} 0.079} & {\color[HTML]{3ED400} 0.249} & {\color[HTML]{E03200} 0.721} & {\color[HTML]{48CA00} 0.125} & {\color[HTML]{4AC800} 0.052} & {\color[HTML]{3BD700} 0.246} & {\color[HTML]{DF3300} 0.638} & {\color[HTML]{41D100} 0.071} & {\color[HTML]{47CB00} 0.03} & {\color[HTML]{35DD00} 0.209} & {\color[HTML]{D63C00} 0.566} \\
gemma2-27b & verb  prob & {\color[HTML]{32E000} 0.415} & {\color[HTML]{987A00} 0.128} & {\color[HTML]{32E000} 0.395} & {\color[HTML]{C34F00} 0.703} & {\color[HTML]{E13200}     -} & {\color[HTML]{E13200}     -} & {\color[HTML]{E13200}     -} & {\color[HTML]{32E100}     -} & {\color[HTML]{E13200}     -} & {\color[HTML]{E13200}     -} & {\color[HTML]{E13200}     -} & {\color[HTML]{32E100}     -} & {\color[HTML]{E13200}     -} & {\color[HTML]{E13200}     -} & {\color[HTML]{E13200}     -} & {\color[HTML]{32E100}     -} \\
gemma2-27b & Calib  -(cluster) & {\color[HTML]{C05200} 0.14} & {\color[HTML]{A17100} 0.118} & {\color[HTML]{D24000} 0.235} & {\color[HTML]{5AB800} 0.639} & {\color[HTML]{4CC600} 0.146} & {\color[HTML]{40D200} 0.125} & {\color[HTML]{3FD300} 0.236} & {\color[HTML]{D93900} 0.645} & {\color[HTML]{47CB00} 0.131} & {\color[HTML]{43CF00} 0.104} & {\color[HTML]{3CD600} 0.238} & {\color[HTML]{E03200} 0.654} & {\color[HTML]{3DD500} 0.097} & {\color[HTML]{3ED400} 0.096} & {\color[HTML]{35DD00} 0.208} & {\color[HTML]{DD3500} 0.639} \\
gemma2-27b & Calib  - & {\color[HTML]{D53D00} 0.1} & {\color[HTML]{C84A00} 0.078} & {\color[HTML]{DD3500} 0.224} & {\color[HTML]{55BD00} 0.636} & {\color[HTML]{52C000} 0.1} & {\color[HTML]{47CB00} 0.078} & {\color[HTML]{41D100} 0.227} & {\color[HTML]{D63C00} 0.622} & {\color[HTML]{4EC400} 0.084} & {\color[HTML]{49C900} 0.061} & {\color[HTML]{3ED400} 0.227} & {\color[HTML]{E03200} 0.649} & {\color[HTML]{3ED400} 0.09} & {\color[HTML]{40D200} 0.082} & {\color[HTML]{37DB00} 0.196} & {\color[HTML]{E03200} 0.668} \\
gemma2-27b & Calib-5 & {\color[HTML]{D93900} 0.092} & {\color[HTML]{C25000} 0.084} & {\color[HTML]{E03200} 0.221} & {\color[HTML]{57BB00} 0.637} & {\color[HTML]{53BF00} 0.098} & {\color[HTML]{47CB00} 0.076} & {\color[HTML]{41D100} 0.221} & {\color[HTML]{D93900} 0.652} & {\color[HTML]{4EC400} 0.086} & {\color[HTML]{46CC00} 0.081} & {\color[HTML]{3ED400} 0.226} & {\color[HTML]{E03200} 0.645} & {\color[HTML]{3FD300} 0.085} & {\color[HTML]{43CF00} 0.058} & {\color[HTML]{37DB00} 0.196} & {\color[HTML]{DF3300} 0.652} \\
gemma2-27b & Calib-5 + PS & {\color[HTML]{D33F00} 0.104} & {\color[HTML]{D83A00} 0.061} & {\color[HTML]{D33F00} 0.234} & {\color[HTML]{4FC300} 0.632} & {\color[HTML]{50C200} 0.118} & {\color[HTML]{4AC800} 0.055} & {\color[HTML]{40D200} 0.234} & {\color[HTML]{D93900} 0.652} & {\color[HTML]{4DC500} 0.089} & {\color[HTML]{49C900} 0.058} & {\color[HTML]{3DD500} 0.235} & {\color[HTML]{E03200} 0.645} & {\color[HTML]{40D200} 0.077} & {\color[HTML]{43CF00} 0.061} & {\color[HTML]{36DC00} 0.201} & {\color[HTML]{DF3300} 0.652} \\
gemma2-27b & bce-auc  small  bert  is  5 & {\color[HTML]{D93900} 0.092} & {\color[HTML]{C25000} 0.084} & {\color[HTML]{E03200} 0.221} & {\color[HTML]{57BB00} 0.637} & {\color[HTML]{53BF00} 0.097} & {\color[HTML]{48CA00} 0.073} & {\color[HTML]{41D100} 0.221} & {\color[HTML]{DA3800} 0.653} & {\color[HTML]{4EC400} 0.085} & {\color[HTML]{47CB00} 0.076} & {\color[HTML]{3ED400} 0.225} & {\color[HTML]{E03200} 0.646} & {\color[HTML]{3FD300} 0.085} & {\color[HTML]{43CF00} 0.063} & {\color[HTML]{37DB00} 0.196} & {\color[HTML]{DF3300} 0.65} \\
gemma2-27b & auc  small  bert  is  5 & {\color[HTML]{928000} 0.228} & {\color[HTML]{51C100} 0.202} & {\color[HTML]{A46E00} 0.281} & {\color[HTML]{52C000} 0.634} & {\color[HTML]{44CE00} 0.21} & {\color[HTML]{37DB00} 0.191} & {\color[HTML]{3AD800} 0.275} & {\color[HTML]{D93900} 0.643} & {\color[HTML]{3BD700} 0.222} & {\color[HTML]{34DE00} 0.205} & {\color[HTML]{37DB00} 0.278} & {\color[HTML]{DF3300} 0.637} & {\color[HTML]{32E000} 0.177} & {\color[HTML]{32E000} 0.178} & {\color[HTML]{32E000} 0.227} & {\color[HTML]{E03200} 0.66} \\
gemma2-27b & (focal)Calib-5 & {\color[HTML]{D83A00} 0.093} & {\color[HTML]{C44E00} 0.082} & {\color[HTML]{DE3400} 0.223} & {\color[HTML]{57BB00} 0.637} & {\color[HTML]{53BF00} 0.091} & {\color[HTML]{48CA00} 0.075} & {\color[HTML]{42D000} 0.219} & {\color[HTML]{DA3800} 0.656} & {\color[HTML]{4DC500} 0.092} & {\color[HTML]{46CC00} 0.085} & {\color[HTML]{3ED400} 0.224} & {\color[HTML]{E03200} 0.652} & {\color[HTML]{3FD300} 0.087} & {\color[HTML]{42D000} 0.068} & {\color[HTML]{36DC00} 0.199} & {\color[HTML]{DE3400} 0.647} \\
gemma2-27b & auc  one  bert  is  1 & {\color[HTML]{AE6400} 0.175} & {\color[HTML]{71A100} 0.169} & {\color[HTML]{B75B00} 0.262} & {\color[HTML]{32E100} 0.614} & {\color[HTML]{4CC600} 0.15} & {\color[HTML]{3CD600} 0.156} & {\color[HTML]{3DD500} 0.256} & {\color[HTML]{D73B00} 0.625} & {\color[HTML]{40D200} 0.188} & {\color[HTML]{3CD600} 0.151} & {\color[HTML]{39D900} 0.265} & {\color[HTML]{DF3300} 0.643} & {\color[HTML]{36DC00} 0.15} & {\color[HTML]{36DC00} 0.145} & {\color[HTML]{33DF00} 0.223} & {\color[HTML]{E03200} 0.664} \\
gemma2-27b & focal  one  bert  is  1 & {\color[HTML]{E13200} 0.077} & {\color[HTML]{DF3300} 0.054} & {\color[HTML]{E13200} 0.22} & {\color[HTML]{45CD00} 0.626} & {\color[HTML]{54BE00} 0.084} & {\color[HTML]{48CA00} 0.075} & {\color[HTML]{41D100} 0.222} & {\color[HTML]{D83A00} 0.635} & {\color[HTML]{4FC300} 0.073} & {\color[HTML]{4AC800} 0.056} & {\color[HTML]{3ED400} 0.224} & {\color[HTML]{E03200} 0.645} & {\color[HTML]{41D100} 0.074} & {\color[HTML]{43CF00} 0.06} & {\color[HTML]{37DB00} 0.193} & {\color[HTML]{E03200} 0.665} \\
\hline
Llama3-70b & LLM Prob. & {\color[HTML]{3AD800} 0.321} & {\color[HTML]{32E000} 0.251} & {\color[HTML]{32E000} 0.339} & {\color[HTML]{D83A00} 0.681} & {\color[HTML]{32E000} 0.35} & {\color[HTML]{32E000} 0.253} & {\color[HTML]{32E000} 0.35} & {\color[HTML]{E03200} 0.702} & {\color[HTML]{32E000} 0.292} & {\color[HTML]{32E000} 0.222} & {\color[HTML]{32E000} 0.322} & {\color[HTML]{DC3600} 0.607} & {\color[HTML]{32E000} 0.168} & {\color[HTML]{39D900} 0.091} & {\color[HTML]{32E000} 0.251} & {\color[HTML]{D04200} 0.554} \\
Llama3-70b & LLM Prob + PS & {\color[HTML]{967C00} 0.194} & {\color[HTML]{BB5700} 0.089} & {\color[HTML]{A56D00} 0.271} & {\color[HTML]{D63C00} 0.68} & {\color[HTML]{4BC700} 0.157} & {\color[HTML]{4CC600} 0.066} & {\color[HTML]{3ED400} 0.254} & {\color[HTML]{E03200} 0.702} & {\color[HTML]{4CC600} 0.099} & {\color[HTML]{4EC400} 0.021} & {\color[HTML]{3CD600} 0.243} & {\color[HTML]{DC3600} 0.607} & {\color[HTML]{3FD300} 0.081} & {\color[HTML]{44CE00} 0.02} & {\color[HTML]{35DD00} 0.225} & {\color[HTML]{D04200} 0.554} \\
Llama3-70b & verb  prob & {\color[HTML]{32E000} 0.333} & {\color[HTML]{CD4500} 0.068} & {\color[HTML]{3AD800} 0.334} & {\color[HTML]{E03200} 0.685} & {\color[HTML]{E13200}     -} & {\color[HTML]{E13200}     -} & {\color[HTML]{E13200}     -} & {\color[HTML]{32E100}     -} & {\color[HTML]{E13200}     -} & {\color[HTML]{E13200}     -} & {\color[HTML]{E13200}     -} & {\color[HTML]{32E100}     -} & {\color[HTML]{E13200}     -} & {\color[HTML]{E13200}     -} & {\color[HTML]{E13200}     -} & {\color[HTML]{32E100}     -} \\
Llama3-70b & Calib  -(cluster) & {\color[HTML]{AD6500} 0.163} & {\color[HTML]{9A7800} 0.128} & {\color[HTML]{C25000} 0.254} & {\color[HTML]{4DC500} 0.616} & {\color[HTML]{4CC600} 0.144} & {\color[HTML]{44CE00} 0.118} & {\color[HTML]{40D200} 0.242} & {\color[HTML]{DB3700} 0.646} & {\color[HTML]{45CD00} 0.145} & {\color[HTML]{41D100} 0.113} & {\color[HTML]{3BD700} 0.25} & {\color[HTML]{DE3400} 0.628} & {\color[HTML]{3BD700} 0.113} & {\color[HTML]{39D900} 0.09} & {\color[HTML]{36DC00} 0.217} & {\color[HTML]{DC3600} 0.674} \\
Llama3-70b & Calib  - & {\color[HTML]{D24000} 0.112} & {\color[HTML]{C44E00} 0.078} & {\color[HTML]{DA3800} 0.24} & {\color[HTML]{32E100} 0.603} & {\color[HTML]{51C100} 0.108} & {\color[HTML]{49C900} 0.082} & {\color[HTML]{41D100} 0.233} & {\color[HTML]{DA3800} 0.637} & {\color[HTML]{4BC700} 0.106} & {\color[HTML]{46CC00} 0.076} & {\color[HTML]{3DD500} 0.237} & {\color[HTML]{DE3400} 0.625} & {\color[HTML]{40D200} 0.075} & {\color[HTML]{3CD600} 0.069} & {\color[HTML]{39D900} 0.198} & {\color[HTML]{DF3300} 0.703} \\
Llama3-70b & Calib-5 & {\color[HTML]{D33F00} 0.11} & {\color[HTML]{B85A00} 0.093} & {\color[HTML]{E13200} 0.236} & {\color[HTML]{838F00} 0.641} & {\color[HTML]{51C100} 0.105} & {\color[HTML]{4CC600} 0.065} & {\color[HTML]{41D100} 0.229} & {\color[HTML]{DC3600} 0.656} & {\color[HTML]{4BC700} 0.104} & {\color[HTML]{46CC00} 0.08} & {\color[HTML]{3ED400} 0.23} & {\color[HTML]{E03200} 0.649} & {\color[HTML]{41D100} 0.073} & {\color[HTML]{3FD300} 0.05} & {\color[HTML]{39D900} 0.195} & {\color[HTML]{E03200} 0.709} \\
Llama3-70b & Calib-5 + PS & {\color[HTML]{E13200} 0.092} & {\color[HTML]{E13200} 0.045} & {\color[HTML]{E13200} 0.236} & {\color[HTML]{5CB600} 0.623} & {\color[HTML]{51C100} 0.107} & {\color[HTML]{4EC400} 0.049} & {\color[HTML]{40D200} 0.235} & {\color[HTML]{DC3600} 0.656} & {\color[HTML]{4FC300} 0.071} & {\color[HTML]{49C900} 0.06} & {\color[HTML]{3ED400} 0.231} & {\color[HTML]{E03200} 0.649} & {\color[HTML]{3DD500} 0.097} & {\color[HTML]{3AD800} 0.085} & {\color[HTML]{38DA00} 0.206} & {\color[HTML]{E03200} 0.709} \\
Llama3-70b & bce-auc  small  bert  is  5 & {\color[HTML]{D33F00} 0.11} & {\color[HTML]{B85A00} 0.093} & {\color[HTML]{E13200} 0.236} & {\color[HTML]{838F00} 0.641} & {\color[HTML]{51C100} 0.105} & {\color[HTML]{4CC600} 0.063} & {\color[HTML]{41D100} 0.228} & {\color[HTML]{DC3600} 0.656} & {\color[HTML]{4BC700} 0.102} & {\color[HTML]{46CC00} 0.081} & {\color[HTML]{3ED400} 0.229} & {\color[HTML]{E03200} 0.648} & {\color[HTML]{41D100} 0.072} & {\color[HTML]{3FD300} 0.052} & {\color[HTML]{39D900} 0.194} & {\color[HTML]{E03200} 0.711} \\
Llama3-70b & auc  small  bert  is  5 & {\color[HTML]{7D9500} 0.229} & {\color[HTML]{5CB600} 0.201} & {\color[HTML]{8A8800} 0.287} & {\color[HTML]{60B200} 0.625} & {\color[HTML]{43CF00} 0.218} & {\color[HTML]{39D900} 0.196} & {\color[HTML]{3AD800} 0.281} & {\color[HTML]{DB3700} 0.645} & {\color[HTML]{39D900} 0.234} & {\color[HTML]{34DE00} 0.202} & {\color[HTML]{37DB00} 0.281} & {\color[HTML]{DF3300} 0.633} & {\color[HTML]{32E000} 0.174} & {\color[HTML]{32E000} 0.137} & {\color[HTML]{35DD00} 0.227} & {\color[HTML]{E03200} 0.714} \\
Llama3-70b & (focal)Calib-5 & {\color[HTML]{D43E00} 0.109} & {\color[HTML]{BF5300} 0.085} & {\color[HTML]{DF3300} 0.237} & {\color[HTML]{7A9800} 0.637} & {\color[HTML]{52C000} 0.096} & {\color[HTML]{4DC500} 0.058} & {\color[HTML]{42D000} 0.226} & {\color[HTML]{DC3600} 0.659} & {\color[HTML]{4BC700} 0.104} & {\color[HTML]{46CC00} 0.076} & {\color[HTML]{3ED400} 0.23} & {\color[HTML]{E03200} 0.651} & {\color[HTML]{3ED400} 0.087} & {\color[HTML]{40D200} 0.04} & {\color[HTML]{39D900} 0.2} & {\color[HTML]{DF3300} 0.697} \\
Llama3-70b & auc  one  bert  is  1 & {\color[HTML]{987A00} 0.192} & {\color[HTML]{69A900} 0.186} & {\color[HTML]{9D7500} 0.276} & {\color[HTML]{34DE00} 0.604} & {\color[HTML]{49C900} 0.172} & {\color[HTML]{3ED400} 0.162} & {\color[HTML]{3DD500} 0.264} & {\color[HTML]{D93900} 0.63} & {\color[HTML]{40D200} 0.185} & {\color[HTML]{3AD800} 0.166} & {\color[HTML]{39D900} 0.265} & {\color[HTML]{DE3400} 0.63} & {\color[HTML]{35DD00} 0.153} & {\color[HTML]{33DF00} 0.125} & {\color[HTML]{36DC00} 0.221} & {\color[HTML]{E03200} 0.707} \\
Llama3-70b & focal  one  bert  is  1 & {\color[HTML]{DF3300} 0.094} & {\color[HTML]{CA4800} 0.072} & {\color[HTML]{DD3500} 0.238} & {\color[HTML]{36DC00} 0.605} & {\color[HTML]{53BF00} 0.094} & {\color[HTML]{4BC700} 0.073} & {\color[HTML]{41D100} 0.229} & {\color[HTML]{DB3700} 0.646} & {\color[HTML]{4DC500} 0.092} & {\color[HTML]{48CA00} 0.065} & {\color[HTML]{3DD500} 0.235} & {\color[HTML]{DE3400} 0.627} & {\color[HTML]{41D100} 0.073} & {\color[HTML]{3ED400} 0.053} & {\color[HTML]{39D900} 0.196} & {\color[HTML]{DF3300} 0.7} \\
\hline
Llama3.1-70b & LLM Prob. & {\color[HTML]{8D8500} 0.203} & {\color[HTML]{38DA00} 0.186} & {\color[HTML]{A66C00} 0.267} & {\color[HTML]{DC3600} 0.695} & {\color[HTML]{34DE00} 0.217} & {\color[HTML]{34DE00} 0.189} & {\color[HTML]{35DD00} 0.268} & {\color[HTML]{E03200} 0.701} & {\color[HTML]{39D900} 0.181} & {\color[HTML]{38DA00} 0.167} & {\color[HTML]{34DE00} 0.264} & {\color[HTML]{DE3400} 0.636} & {\color[HTML]{3CD600} 0.096} & {\color[HTML]{3ED400} 0.071} & {\color[HTML]{34DE00} 0.197} & {\color[HTML]{DC3600} 0.654} \\
Llama3.1-70b & LLM Prob + PS & {\color[HTML]{A66C00} 0.16} & {\color[HTML]{C34F00} 0.061} & {\color[HTML]{B16100} 0.259} & {\color[HTML]{C15100} 0.683} & {\color[HTML]{40D200} 0.135} & {\color[HTML]{47CB00} 0.062} & {\color[HTML]{39D900} 0.238} & {\color[HTML]{E03200} 0.701} & {\color[HTML]{46CC00} 0.086} & {\color[HTML]{49C900} 0.051} & {\color[HTML]{38DA00} 0.235} & {\color[HTML]{DE3400} 0.636} & {\color[HTML]{3BD700} 0.106} & {\color[HTML]{41D100} 0.053} & {\color[HTML]{33DF00} 0.201} & {\color[HTML]{DC3600} 0.654} \\
Llama3.1-70b & verb  prob & {\color[HTML]{32E000} 0.356} & {\color[HTML]{8A8800} 0.112} & {\color[HTML]{32E000} 0.348} & {\color[HTML]{E03200} 0.697} & {\color[HTML]{E13200}     -} & {\color[HTML]{E13200}     -} & {\color[HTML]{E13200}     -} & {\color[HTML]{32E100}     -} & {\color[HTML]{E13200}     -} & {\color[HTML]{E13200}     -} & {\color[HTML]{E13200}     -} & {\color[HTML]{32E100}     -} & {\color[HTML]{E13200}     -} & {\color[HTML]{E13200}     -} & {\color[HTML]{E13200}     -} & {\color[HTML]{32E100}     -} \\
Llama3.1-70b & Calib  -(cluster) & {\color[HTML]{B55D00} 0.135} & {\color[HTML]{858D00} 0.117} & {\color[HTML]{C84A00} 0.243} & {\color[HTML]{6DA500} 0.646} & {\color[HTML]{3FD300} 0.146} & {\color[HTML]{3ED400} 0.123} & {\color[HTML]{37DB00} 0.255} & {\color[HTML]{D73B00} 0.608} & {\color[HTML]{40D200} 0.135} & {\color[HTML]{41D100} 0.107} & {\color[HTML]{37DB00} 0.238} & {\color[HTML]{E03200} 0.657} & {\color[HTML]{3BD700} 0.1} & {\color[HTML]{3CD600} 0.087} & {\color[HTML]{34DE00} 0.195} & {\color[HTML]{DE3400} 0.667} \\
Llama3.1-70b & Calib  - & {\color[HTML]{CE4400} 0.093} & {\color[HTML]{B85A00} 0.071} & {\color[HTML]{D43E00} 0.235} & {\color[HTML]{32E100} 0.62} & {\color[HTML]{45CD00} 0.1} & {\color[HTML]{46CC00} 0.066} & {\color[HTML]{39D900} 0.237} & {\color[HTML]{D73B00} 0.608} & {\color[HTML]{46CC00} 0.092} & {\color[HTML]{47CB00} 0.064} & {\color[HTML]{39D900} 0.225} & {\color[HTML]{E03200} 0.652} & {\color[HTML]{40D200} 0.07} & {\color[HTML]{3FD300} 0.069} & {\color[HTML]{36DC00} 0.184} & {\color[HTML]{E03200} 0.688} \\
Llama3.1-70b & Calib-5 & {\color[HTML]{C84A00} 0.104} & {\color[HTML]{B95900} 0.07} & {\color[HTML]{D83A00} 0.232} & {\color[HTML]{868C00} 0.657} & {\color[HTML]{43CF00} 0.112} & {\color[HTML]{45CD00} 0.073} & {\color[HTML]{39D900} 0.239} & {\color[HTML]{D93900} 0.627} & {\color[HTML]{46CC00} 0.087} & {\color[HTML]{45CD00} 0.074} & {\color[HTML]{38DA00} 0.23} & {\color[HTML]{E03200} 0.649} & {\color[HTML]{40D200} 0.068} & {\color[HTML]{41D100} 0.055} & {\color[HTML]{36DC00} 0.184} & {\color[HTML]{E03200} 0.689} \\
Llama3.1-70b & Calib-5 + PS & {\color[HTML]{D73B00} 0.078} & {\color[HTML]{E13200} 0.034} & {\color[HTML]{D14100} 0.237} & {\color[HTML]{38DA00} 0.623} & {\color[HTML]{47CB00} 0.085} & {\color[HTML]{48CA00} 0.051} & {\color[HTML]{3AD800} 0.234} & {\color[HTML]{D93900} 0.627} & {\color[HTML]{4AC800} 0.062} & {\color[HTML]{46CC00} 0.068} & {\color[HTML]{38DA00} 0.23} & {\color[HTML]{E03200} 0.649} & {\color[HTML]{3BD700} 0.104} & {\color[HTML]{3ED400} 0.075} & {\color[HTML]{34DE00} 0.196} & {\color[HTML]{E03200} 0.689} \\
Llama3.1-70b & bce-auc  small  bert  is  5 & {\color[HTML]{C84A00} 0.104} & {\color[HTML]{B95900} 0.07} & {\color[HTML]{D83A00} 0.232} & {\color[HTML]{868C00} 0.657} & {\color[HTML]{44CE00} 0.108} & {\color[HTML]{45CD00} 0.071} & {\color[HTML]{39D900} 0.239} & {\color[HTML]{D93900} 0.627} & {\color[HTML]{46CC00} 0.087} & {\color[HTML]{45CD00} 0.079} & {\color[HTML]{38DA00} 0.23} & {\color[HTML]{E03200} 0.648} & {\color[HTML]{40D200} 0.068} & {\color[HTML]{41D100} 0.056} & {\color[HTML]{36DC00} 0.183} & {\color[HTML]{E03200} 0.691} \\
Llama3.1-70b & auc  small  bert  is  5 & {\color[HTML]{829000} 0.221} & {\color[HTML]{32E000} 0.192} & {\color[HTML]{928000} 0.281} & {\color[HTML]{6AA800} 0.645} & {\color[HTML]{32E000} 0.238} & {\color[HTML]{32E000} 0.209} & {\color[HTML]{32E000} 0.296} & {\color[HTML]{D73B00} 0.611} & {\color[HTML]{32E000} 0.234} & {\color[HTML]{32E000} 0.212} & {\color[HTML]{32E000} 0.281} & {\color[HTML]{DD3500} 0.626} & {\color[HTML]{32E000} 0.166} & {\color[HTML]{32E000} 0.155} & {\color[HTML]{32E000} 0.214} & {\color[HTML]{E03200} 0.696} \\
Llama3.1-70b & (focal)Calib-5 & {\color[HTML]{CA4800} 0.1} & {\color[HTML]{B45E00} 0.074} & {\color[HTML]{D63C00} 0.233} & {\color[HTML]{838F00} 0.656} & {\color[HTML]{45CD00} 0.102} & {\color[HTML]{46CC00} 0.07} & {\color[HTML]{39D900} 0.238} & {\color[HTML]{D93900} 0.624} & {\color[HTML]{45CD00} 0.094} & {\color[HTML]{45CD00} 0.077} & {\color[HTML]{39D900} 0.228} & {\color[HTML]{E03200} 0.656} & {\color[HTML]{41D100} 0.065} & {\color[HTML]{41D100} 0.056} & {\color[HTML]{36DC00} 0.186} & {\color[HTML]{DF3300} 0.686} \\
Llama3.1-70b & auc  one  bert  is  1 & {\color[HTML]{9B7700} 0.179} & {\color[HTML]{6BA700} 0.14} & {\color[HTML]{AA6800} 0.264} & {\color[HTML]{838F00} 0.656} & {\color[HTML]{3AD800} 0.181} & {\color[HTML]{39D900} 0.158} & {\color[HTML]{35DD00} 0.272} & {\color[HTML]{D73B00} 0.607} & {\color[HTML]{32E000} 0.227} & {\color[HTML]{39D900} 0.163} & {\color[HTML]{32E000} 0.275} & {\color[HTML]{DF3300} 0.641} & {\color[HTML]{36DC00} 0.135} & {\color[HTML]{36DC00} 0.126} & {\color[HTML]{33DF00} 0.204} & {\color[HTML]{DF3300} 0.684} \\
Llama3.1-70b & focal  one  bert  is  1 & {\color[HTML]{E13200} 0.062} & {\color[HTML]{CE4400} 0.051} & {\color[HTML]{E13200} 0.226} & {\color[HTML]{6FA300} 0.647} & {\color[HTML]{48CA00} 0.08} & {\color[HTML]{48CA00} 0.052} & {\color[HTML]{3AD800} 0.236} & {\color[HTML]{D63C00} 0.603} & {\color[HTML]{47CB00} 0.082} & {\color[HTML]{48CA00} 0.053} & {\color[HTML]{39D900} 0.223} & {\color[HTML]{E03200} 0.655} & {\color[HTML]{42D000} 0.053} & {\color[HTML]{41D100} 0.053} & {\color[HTML]{36DC00} 0.183} & {\color[HTML]{DF3300} 0.686} \\
\hline
Qwen2-72b & LLM Prob. & {\color[HTML]{3ED400} 0.339} & {\color[HTML]{32E000} 0.247} & {\color[HTML]{36DC00} 0.348} & {\color[HTML]{B85A00} 0.69} & {\color[HTML]{32E000} 0.389} & {\color[HTML]{32E000} 0.24} & {\color[HTML]{32E000} 0.376} & {\color[HTML]{E03200} 0.731} & {\color[HTML]{32E000} 0.275} & {\color[HTML]{32E000} 0.229} & {\color[HTML]{32E000} 0.316} & {\color[HTML]{DA3800} 0.597} & {\color[HTML]{39D900} 0.129} & {\color[HTML]{3FD300} 0.077} & {\color[HTML]{33DF00} 0.22} & {\color[HTML]{DA3800} 0.636} \\
Qwen2-72b & LLM Prob + PS & {\color[HTML]{AC6600} 0.159} & {\color[HTML]{A96900} 0.098} & {\color[HTML]{C44E00} 0.252} & {\color[HTML]{D33F00} 0.71} & {\color[HTML]{4DC500} 0.173} & {\color[HTML]{4CC600} 0.05} & {\color[HTML]{40D200} 0.259} & {\color[HTML]{E03200} 0.731} & {\color[HTML]{4AC800} 0.097} & {\color[HTML]{4EC400} 0.03} & {\color[HTML]{3BD700} 0.243} & {\color[HTML]{DA3800} 0.597} & {\color[HTML]{3CD600} 0.11} & {\color[HTML]{42D000} 0.055} & {\color[HTML]{34DE00} 0.219} & {\color[HTML]{DA3800} 0.636} \\
Qwen2-72b & verb  prob & {\color[HTML]{32E000} 0.359} & {\color[HTML]{C84A00} 0.059} & {\color[HTML]{32E000} 0.351} & {\color[HTML]{E03200} 0.72} & {\color[HTML]{E13200}     -} & {\color[HTML]{E13200}     -} & {\color[HTML]{E13200}     -} & {\color[HTML]{32E100}     -} & {\color[HTML]{E13200}     -} & {\color[HTML]{E13200}     -} & {\color[HTML]{E13200}     -} & {\color[HTML]{32E100}     -} & {\color[HTML]{E13200}     -} & {\color[HTML]{E13200}     -} & {\color[HTML]{E13200}     -} & {\color[HTML]{32E100}     -} \\
Qwen2-72b & Calib  -(cluster) & {\color[HTML]{B06200} 0.153} & {\color[HTML]{8C8600} 0.134} & {\color[HTML]{C74B00} 0.25} & {\color[HTML]{5CB600} 0.621} & {\color[HTML]{52C000} 0.135} & {\color[HTML]{43CF00} 0.117} & {\color[HTML]{42D000} 0.243} & {\color[HTML]{D73B00} 0.633} & {\color[HTML]{44CE00} 0.138} & {\color[HTML]{40D200} 0.126} & {\color[HTML]{3BD700} 0.247} & {\color[HTML]{DE3400} 0.629} & {\color[HTML]{3FD300} 0.086} & {\color[HTML]{3ED400} 0.085} & {\color[HTML]{35DD00} 0.212} & {\color[HTML]{DB3700} 0.64} \\
Qwen2-72b & Calib  - & {\color[HTML]{DD3500} 0.078} & {\color[HTML]{C64C00} 0.061} & {\color[HTML]{E13200} 0.233} & {\color[HTML]{34DE00} 0.591} & {\color[HTML]{59B900} 0.077} & {\color[HTML]{4DC500} 0.043} & {\color[HTML]{44CE00} 0.231} & {\color[HTML]{D63C00} 0.623} & {\color[HTML]{4CC600} 0.082} & {\color[HTML]{48CA00} 0.074} & {\color[HTML]{3DD500} 0.227} & {\color[HTML]{E03200} 0.65} & {\color[HTML]{3FD300} 0.088} & {\color[HTML]{3ED400} 0.079} & {\color[HTML]{36DC00} 0.201} & {\color[HTML]{DE3400} 0.674} \\
Qwen2-72b & Calib-5 & {\color[HTML]{D63C00} 0.09} & {\color[HTML]{B26000} 0.086} & {\color[HTML]{DB3700} 0.237} & {\color[HTML]{54BE00} 0.615} & {\color[HTML]{57BB00} 0.092} & {\color[HTML]{49C900} 0.07} & {\color[HTML]{44CE00} 0.232} & {\color[HTML]{D63C00} 0.632} & {\color[HTML]{4BC700} 0.089} & {\color[HTML]{47CB00} 0.075} & {\color[HTML]{3DD500} 0.228} & {\color[HTML]{E03200} 0.657} & {\color[HTML]{41D100} 0.077} & {\color[HTML]{43CF00} 0.05} & {\color[HTML]{37DB00} 0.197} & {\color[HTML]{E03200} 0.694} \\
Qwen2-72b & Calib-5 + PS & {\color[HTML]{DA3800} 0.083} & {\color[HTML]{E13200} 0.028} & {\color[HTML]{DC3600} 0.236} & {\color[HTML]{43CF00} 0.602} & {\color[HTML]{56BC00} 0.099} & {\color[HTML]{4DC500} 0.042} & {\color[HTML]{43CF00} 0.238} & {\color[HTML]{D63C00} 0.632} & {\color[HTML]{4EC400} 0.069} & {\color[HTML]{4AC800} 0.055} & {\color[HTML]{3DD500} 0.231} & {\color[HTML]{E03200} 0.657} & {\color[HTML]{3FD300} 0.09} & {\color[HTML]{3ED400} 0.081} & {\color[HTML]{35DD00} 0.206} & {\color[HTML]{E03200} 0.694} \\
Qwen2-72b & bce-auc  small  bert  is  5 & {\color[HTML]{D63C00} 0.09} & {\color[HTML]{B26000} 0.086} & {\color[HTML]{DB3700} 0.237} & {\color[HTML]{54BE00} 0.615} & {\color[HTML]{57BB00} 0.091} & {\color[HTML]{49C900} 0.07} & {\color[HTML]{44CE00} 0.232} & {\color[HTML]{D73B00} 0.633} & {\color[HTML]{4BC700} 0.087} & {\color[HTML]{48CA00} 0.073} & {\color[HTML]{3DD500} 0.228} & {\color[HTML]{E03200} 0.656} & {\color[HTML]{41D100} 0.072} & {\color[HTML]{42D000} 0.052} & {\color[HTML]{37DB00} 0.197} & {\color[HTML]{E03200} 0.694} \\
Qwen2-72b & auc  small  bert  is  5 & {\color[HTML]{739F00} 0.252} & {\color[HTML]{39D900} 0.237} & {\color[HTML]{739F00} 0.307} & {\color[HTML]{3FD300} 0.599} & {\color[HTML]{45CD00} 0.237} & {\color[HTML]{33DF00} 0.226} & {\color[HTML]{3CD600} 0.295} & {\color[HTML]{D53D00} 0.62} & {\color[HTML]{3AD800} 0.214} & {\color[HTML]{36DC00} 0.199} & {\color[HTML]{37DB00} 0.275} & {\color[HTML]{DF3300} 0.647} & {\color[HTML]{32E000} 0.178} & {\color[HTML]{32E000} 0.165} & {\color[HTML]{32E000} 0.234} & {\color[HTML]{E03200} 0.698} \\
Qwen2-72b & (focal)Calib-5 & {\color[HTML]{CF4300} 0.102} & {\color[HTML]{AD6500} 0.092} & {\color[HTML]{D83A00} 0.239} & {\color[HTML]{4AC800} 0.607} & {\color[HTML]{58BA00} 0.082} & {\color[HTML]{49C900} 0.071} & {\color[HTML]{44CE00} 0.231} & {\color[HTML]{D73B00} 0.633} & {\color[HTML]{4BC700} 0.087} & {\color[HTML]{46CC00} 0.083} & {\color[HTML]{3DD500} 0.227} & {\color[HTML]{E03200} 0.656} & {\color[HTML]{3FD300} 0.084} & {\color[HTML]{43CF00} 0.051} & {\color[HTML]{36DC00} 0.199} & {\color[HTML]{E03200} 0.691} \\
Qwen2-72b & auc  one  bert  is  1 & {\color[HTML]{8D8500} 0.209} & {\color[HTML]{779B00} 0.16} & {\color[HTML]{9E7400} 0.278} & {\color[HTML]{40D200} 0.6} & {\color[HTML]{4CC600} 0.181} & {\color[HTML]{3CD600} 0.165} & {\color[HTML]{3FD300} 0.266} & {\color[HTML]{D43E00} 0.607} & {\color[HTML]{40D200} 0.173} & {\color[HTML]{3CD600} 0.156} & {\color[HTML]{39D900} 0.26} & {\color[HTML]{DE3400} 0.636} & {\color[HTML]{34DE00} 0.161} & {\color[HTML]{33DF00} 0.153} & {\color[HTML]{32E000} 0.233} & {\color[HTML]{DE3400} 0.677} \\
Qwen2-72b & focal  one  bert  is  1 & {\color[HTML]{E13200} 0.073} & {\color[HTML]{C54D00} 0.063} & {\color[HTML]{DE3400} 0.235} & {\color[HTML]{32E100} 0.589} & {\color[HTML]{5BB700} 0.059} & {\color[HTML]{4FC300} 0.034} & {\color[HTML]{44CE00} 0.227} & {\color[HTML]{D53D00} 0.615} & {\color[HTML]{4DC500} 0.076} & {\color[HTML]{4AC800} 0.055} & {\color[HTML]{3DD500} 0.226} & {\color[HTML]{E03200} 0.649} & {\color[HTML]{40D200} 0.08} & {\color[HTML]{40D200} 0.067} & {\color[HTML]{36DC00} 0.201} & {\color[HTML]{DE3400} 0.671} \\
\hline
Mixtral-8x7B & LLM Prob. & {\color[HTML]{32E000} 0.356} & {\color[HTML]{32E000} 0.256} & {\color[HTML]{32E000} 0.362} & {\color[HTML]{E03200} 0.663} & {\color[HTML]{32E000} 0.298} & {\color[HTML]{3BD700} 0.167} & {\color[HTML]{32E000} 0.319} & {\color[HTML]{E03200} 0.654} & {\color[HTML]{32E000} 0.319} & {\color[HTML]{32E000} 0.231} & {\color[HTML]{32E000} 0.337} & {\color[HTML]{DE3400} 0.602} & {\color[HTML]{32E000} 0.221} & {\color[HTML]{40D200} 0.081} & {\color[HTML]{32E000} 0.288} & {\color[HTML]{D43E00} 0.541} \\
Mixtral-8x7B & LLM Prob + PS & {\color[HTML]{BD5500} 0.127} & {\color[HTML]{DC3600} 0.022} & {\color[HTML]{C74B00} 0.255} & {\color[HTML]{749E00} 0.609} & {\color[HTML]{47CB00} 0.135} & {\color[HTML]{4AC800} 0.064} & {\color[HTML]{3AD800} 0.255} & {\color[HTML]{E03200} 0.654} & {\color[HTML]{4DC500} 0.112} & {\color[HTML]{50C200} 0.013} & {\color[HTML]{3DD500} 0.248} & {\color[HTML]{DE3400} 0.602} & {\color[HTML]{45CD00} 0.09} & {\color[HTML]{4AC800} 0.011} & {\color[HTML]{38DA00} 0.242} & {\color[HTML]{D43E00} 0.541} \\
Mixtral-8x7B & verb  prob & {\color[HTML]{37DB00} 0.347} & {\color[HTML]{9E7400} 0.107} & {\color[HTML]{44CE00} 0.349} & {\color[HTML]{967C00} 0.626} & {\color[HTML]{E13200}     -} & {\color[HTML]{E13200}     -} & {\color[HTML]{E13200}     -} & {\color[HTML]{32E100}     -} & {\color[HTML]{E13200}     -} & {\color[HTML]{E13200}     -} & {\color[HTML]{E13200}     -} & {\color[HTML]{32E100}     -} & {\color[HTML]{E13200}     -} & {\color[HTML]{E13200}     -} & {\color[HTML]{E13200}     -} & {\color[HTML]{32E100}     -} \\
Mixtral-8x7B & Calib  -(cluster) & {\color[HTML]{AC6600} 0.155} & {\color[HTML]{898900} 0.136} & {\color[HTML]{B95900} 0.265} & {\color[HTML]{68AA00} 0.603} & {\color[HTML]{48CA00} 0.133} & {\color[HTML]{42D000} 0.121} & {\color[HTML]{3BD700} 0.251} & {\color[HTML]{DD3500} 0.618} & {\color[HTML]{4DC500} 0.111} & {\color[HTML]{43CF00} 0.108} & {\color[HTML]{3ED400} 0.24} & {\color[HTML]{E03200} 0.625} & {\color[HTML]{3CD600} 0.152} & {\color[HTML]{3DD500} 0.098} & {\color[HTML]{35DD00} 0.259} & {\color[HTML]{DA3800} 0.598} \\
Mixtral-8x7B & Calib  - & {\color[HTML]{D93900} 0.081} & {\color[HTML]{C44E00} 0.055} & {\color[HTML]{DB3700} 0.241} & {\color[HTML]{44CE00} 0.585} & {\color[HTML]{50C200} 0.069} & {\color[HTML]{4BC700} 0.055} & {\color[HTML]{3DD500} 0.23} & {\color[HTML]{DF3300} 0.642} & {\color[HTML]{53BF00} 0.066} & {\color[HTML]{49C900} 0.064} & {\color[HTML]{40D200} 0.227} & {\color[HTML]{E03200} 0.626} & {\color[HTML]{42D000} 0.114} & {\color[HTML]{41D100} 0.07} & {\color[HTML]{38DA00} 0.239} & {\color[HTML]{DD3500} 0.626} \\
Mixtral-8x7B & Calib-5 & {\color[HTML]{C44E00} 0.115} & {\color[HTML]{AF6300} 0.084} & {\color[HTML]{D04200} 0.249} & {\color[HTML]{68AA00} 0.603} & {\color[HTML]{4FC300} 0.08} & {\color[HTML]{48CA00} 0.074} & {\color[HTML]{3BD700} 0.244} & {\color[HTML]{DA3800} 0.595} & {\color[HTML]{52C000} 0.071} & {\color[HTML]{4AC800} 0.061} & {\color[HTML]{3FD300} 0.235} & {\color[HTML]{DE3400} 0.6} & {\color[HTML]{45CD00} 0.087} & {\color[HTML]{44CE00} 0.055} & {\color[HTML]{3AD800} 0.225} & {\color[HTML]{E03200} 0.654} \\
Mixtral-8x7B & Calib-5 + PS & {\color[HTML]{E13200} 0.068} & {\color[HTML]{E13200} 0.016} & {\color[HTML]{D83A00} 0.243} & {\color[HTML]{3CD600} 0.581} & {\color[HTML]{51C100} 0.064} & {\color[HTML]{4EC400} 0.032} & {\color[HTML]{3CD600} 0.241} & {\color[HTML]{DA3800} 0.595} & {\color[HTML]{53BF00} 0.063} & {\color[HTML]{4DC500} 0.037} & {\color[HTML]{3FD300} 0.232} & {\color[HTML]{DE3400} 0.6} & {\color[HTML]{48CA00} 0.068} & {\color[HTML]{44CE00} 0.055} & {\color[HTML]{3AD800} 0.226} & {\color[HTML]{E03200} 0.654} \\
Mixtral-8x7B & bce-auc  small  bert  is  5 & {\color[HTML]{C44E00} 0.115} & {\color[HTML]{AF6300} 0.084} & {\color[HTML]{D04200} 0.249} & {\color[HTML]{68AA00} 0.603} & {\color[HTML]{4FC300} 0.077} & {\color[HTML]{48CA00} 0.075} & {\color[HTML]{3BD700} 0.244} & {\color[HTML]{DA3800} 0.593} & {\color[HTML]{53BF00} 0.07} & {\color[HTML]{4AC800} 0.059} & {\color[HTML]{3FD300} 0.235} & {\color[HTML]{DE3400} 0.602} & {\color[HTML]{46CC00} 0.086} & {\color[HTML]{43CF00} 0.056} & {\color[HTML]{3AD800} 0.224} & {\color[HTML]{E03200} 0.655} \\
Mixtral-8x7B & auc  small  bert  is  5 & {\color[HTML]{69A900} 0.265} & {\color[HTML]{3AD800} 0.245} & {\color[HTML]{769C00} 0.313} & {\color[HTML]{44CE00} 0.585} & {\color[HTML]{36DC00} 0.262} & {\color[HTML]{32E000} 0.235} & {\color[HTML]{32E000} 0.313} & {\color[HTML]{D93900} 0.582} & {\color[HTML]{40D200} 0.213} & {\color[HTML]{3BD700} 0.165} & {\color[HTML]{38DA00} 0.284} & {\color[HTML]{DC3600} 0.582} & {\color[HTML]{32E000} 0.227} & {\color[HTML]{32E000} 0.177} & {\color[HTML]{33DF00} 0.279} & {\color[HTML]{E03200} 0.655} \\
Mixtral-8x7B & (focal)Calib-5 & {\color[HTML]{C34F00} 0.117} & {\color[HTML]{AA6800} 0.091} & {\color[HTML]{CC4600} 0.252} & {\color[HTML]{5AB800} 0.596} & {\color[HTML]{51C100} 0.066} & {\color[HTML]{4AC800} 0.063} & {\color[HTML]{3CD600} 0.24} & {\color[HTML]{DB3700} 0.599} & {\color[HTML]{51C100} 0.081} & {\color[HTML]{48CA00} 0.072} & {\color[HTML]{3FD300} 0.234} & {\color[HTML]{DF3300} 0.611} & {\color[HTML]{46CC00} 0.083} & {\color[HTML]{43CF00} 0.061} & {\color[HTML]{3AD800} 0.226} & {\color[HTML]{E03200} 0.653} \\
Mixtral-8x7B & auc  one  bert  is  1 & {\color[HTML]{848E00} 0.22} & {\color[HTML]{4CC600} 0.22} & {\color[HTML]{997900} 0.288} & {\color[HTML]{32E100} 0.576} & {\color[HTML]{43CF00} 0.169} & {\color[HTML]{3ED400} 0.148} & {\color[HTML]{39D900} 0.26} & {\color[HTML]{DF3300} 0.643} & {\color[HTML]{46CC00} 0.163} & {\color[HTML]{40D200} 0.131} & {\color[HTML]{3BD700} 0.262} & {\color[HTML]{DF3300} 0.615} & {\color[HTML]{3AD800} 0.167} & {\color[HTML]{3DD500} 0.099} & {\color[HTML]{33DF00} 0.277} & {\color[HTML]{DC3600} 0.614} \\
Mixtral-8x7B & focal  one  bert  is  1 & {\color[HTML]{DF3300} 0.071} & {\color[HTML]{CC4600} 0.044} & {\color[HTML]{E13200} 0.237} & {\color[HTML]{4AC800} 0.588} & {\color[HTML]{52C000} 0.058} & {\color[HTML]{4CC600} 0.045} & {\color[HTML]{3ED400} 0.228} & {\color[HTML]{DF3300} 0.642} & {\color[HTML]{55BD00} 0.049} & {\color[HTML]{4DC500} 0.038} & {\color[HTML]{40D200} 0.226} & {\color[HTML]{E03200} 0.618} & {\color[HTML]{43CF00} 0.106} & {\color[HTML]{42D000} 0.066} & {\color[HTML]{38DA00} 0.237} & {\color[HTML]{DE3400} 0.633} \\
\hline


==> tables/text/small_model_results_text.tex <==
llama7 & LLM Prob. & {\color[HTML]{32E000} 0.435} & {\color[HTML]{50C200} 0.223} & {\color[HTML]{37DB00} 0.4} & {\color[HTML]{E03200} 0.71} & {\color[HTML]{32E000} 0.335} & {\color[HTML]{3DD500} 0.161} & {\color[HTML]{32E000} 0.304} & {\color[HTML]{E03200} 0.738} & {\color[HTML]{32E000} 0.323} & {\color[HTML]{38DA00} 0.165} & {\color[HTML]{32E000} 0.337} & {\color[HTML]{DB3700} 0.655} & {\color[HTML]{32E000} 0.442} & {\color[HTML]{47CB00} 0.063} & {\color[HTML]{32E000} 0.418} & {\color[HTML]{D53D00} 0.613} \\
llama7 & LLM Prob + PS & {\color[HTML]{5FB300} 0.338} & {\color[HTML]{DF3300} 0.034} & {\color[HTML]{739F00} 0.334} & {\color[HTML]{6EA400} 0.643} & {\color[HTML]{35DD00} 0.305} & {\color[HTML]{4AC800} 0.072} & {\color[HTML]{36DC00} 0.27} & {\color[HTML]{E03200} 0.739} & {\color[HTML]{41D100} 0.203} & {\color[HTML]{44CE00} 0.085} & {\color[HTML]{3BD700} 0.265} & {\color[HTML]{E03200} 0.707} & {\color[HTML]{47CB00} 0.263} & {\color[HTML]{4BC700} 0.03} & {\color[HTML]{41D100} 0.295} & {\color[HTML]{D53D00} 0.615} \\
llama7 & verb  prob & {\color[HTML]{32E000} 0.436} & {\color[HTML]{D73B00} 0.044} & {\color[HTML]{32E000} 0.406} & {\color[HTML]{5EB400} 0.634} & {\color[HTML]{E13200}     -} & {\color[HTML]{E13200}     -} & {\color[HTML]{E13200}     -} & {\color[HTML]{32E100}     -} & {\color[HTML]{E13200}     -} & {\color[HTML]{E13200}     -} & {\color[HTML]{E13200}     -} & {\color[HTML]{32E100}     -} & {\color[HTML]{E13200}     -} & {\color[HTML]{E13200}     -} & {\color[HTML]{E13200}     -} & {\color[HTML]{32E100}     -} \\
llama7 & Calib  -(cluster) & {\color[HTML]{C25000} 0.129} & {\color[HTML]{AF6300} 0.097} & {\color[HTML]{D43E00} 0.227} & {\color[HTML]{68AA00} 0.64} & {\color[HTML]{4FC300} 0.113} & {\color[HTML]{48CA00} 0.086} & {\color[HTML]{41D100} 0.189} & {\color[HTML]{DB3700} 0.682} & {\color[HTML]{4CC600} 0.125} & {\color[HTML]{40D200} 0.11} & {\color[HTML]{3ED400} 0.24} & {\color[HTML]{DB3700} 0.657} & {\color[HTML]{59B900} 0.114} & {\color[HTML]{46CC00} 0.07} & {\color[HTML]{4AC800} 0.22} & {\color[HTML]{DC3600} 0.679} \\
llama7 & Calib  - & {\color[HTML]{D43E00} 0.089} & {\color[HTML]{CA4800} 0.062} & {\color[HTML]{DB3700} 0.219} & {\color[HTML]{50C200} 0.626} & {\color[HTML]{53BF00} 0.083} & {\color[HTML]{4DC500} 0.051} & {\color[HTML]{41D100} 0.185} & {\color[HTML]{D83A00} 0.658} & {\color[HTML]{50C200} 0.094} & {\color[HTML]{46CC00} 0.072} & {\color[HTML]{3FD300} 0.231} & {\color[HTML]{DA3800} 0.645} & {\color[HTML]{5AB800} 0.107} & {\color[HTML]{46CC00} 0.07} & {\color[HTML]{4AC800} 0.217} & {\color[HTML]{DC3600} 0.683} \\
llama7 & Calib-7 & {\color[HTML]{C84A00} 0.115} & {\color[HTML]{B45E00} 0.091} & {\color[HTML]{D93900} 0.221} & {\color[HTML]{749E00} 0.647} & {\color[HTML]{51C100} 0.093} & {\color[HTML]{4AC800} 0.072} & {\color[HTML]{41D100} 0.191} & {\color[HTML]{DB3700} 0.683} & {\color[HTML]{4EC400} 0.11} & {\color[HTML]{45CD00} 0.077} & {\color[HTML]{40D200} 0.228} & {\color[HTML]{DD3500} 0.672} & {\color[HTML]{5DB500} 0.082} & {\color[HTML]{45CD00} 0.073} & {\color[HTML]{4CC600} 0.205} & {\color[HTML]{DF3300} 0.715} \\
llama7 & Calib-5 + PS & {\color[HTML]{AF6300} 0.168} & {\color[HTML]{E13200} 0.032} & {\color[HTML]{C54D00} 0.243} & {\color[HTML]{4FC300} 0.625} & {\color[HTML]{3FD300} 0.231} & {\color[HTML]{4DC500} 0.046} & {\color[HTML]{3BD700} 0.235} & {\color[HTML]{DB3700} 0.683} & {\color[HTML]{4BC700} 0.13} & {\color[HTML]{45CD00} 0.075} & {\color[HTML]{3DD500} 0.247} & {\color[HTML]{DD3500} 0.672} & {\color[HTML]{53BF00} 0.168} & {\color[HTML]{44CE00} 0.082} & {\color[HTML]{48CA00} 0.238} & {\color[HTML]{DF3300} 0.715} \\
llama7 & bce-auc  small  bert  is  7 & {\color[HTML]{C84A00} 0.115} & {\color[HTML]{B45E00} 0.091} & {\color[HTML]{D93900} 0.221} & {\color[HTML]{749E00} 0.647} & {\color[HTML]{51C100} 0.092} & {\color[HTML]{49C900} 0.075} & {\color[HTML]{41D100} 0.191} & {\color[HTML]{DB3700} 0.683} & {\color[HTML]{4EC400} 0.11} & {\color[HTML]{45CD00} 0.075} & {\color[HTML]{40D200} 0.229} & {\color[HTML]{DD3500} 0.672} & {\color[HTML]{5DB500} 0.081} & {\color[HTML]{45CD00} 0.073} & {\color[HTML]{4CC600} 0.205} & {\color[HTML]{DF3300} 0.715} \\
llama7 & (auc)Calib-7 & {\color[HTML]{829000} 0.265} & {\color[HTML]{32E000} 0.263} & {\color[HTML]{8B8700} 0.307} & {\color[HTML]{67AB00} 0.639} & {\color[HTML]{3BD700} 0.261} & {\color[HTML]{32E000} 0.245} & {\color[HTML]{34DE00} 0.282} & {\color[HTML]{D93900} 0.661} & {\color[HTML]{3ED400} 0.232} & {\color[HTML]{32E000} 0.213} & {\color[HTML]{38DA00} 0.291} & {\color[HTML]{DB3700} 0.654} & {\color[HTML]{4CC600} 0.223} & {\color[HTML]{32E000} 0.209} & {\color[HTML]{45CD00} 0.26} & {\color[HTML]{E03200} 0.726} \\
llama7 & (focal)Calib-7 & {\color[HTML]{C64C00} 0.12} & {\color[HTML]{AC6600} 0.101} & {\color[HTML]{D43E00} 0.227} & {\color[HTML]{48CA00} 0.621} & {\color[HTML]{51C100} 0.098} & {\color[HTML]{4AC800} 0.071} & {\color[HTML]{41D100} 0.191} & {\color[HTML]{DA3800} 0.676} & {\color[HTML]{4FC300} 0.102} & {\color[HTML]{45CD00} 0.077} & {\color[HTML]{40D200} 0.224} & {\color[HTML]{DD3500} 0.673} & {\color[HTML]{5DB500} 0.085} & {\color[HTML]{46CC00} 0.07} & {\color[HTML]{4CC600} 0.203} & {\color[HTML]{E03200} 0.717} \\
llama7 & auc  one  bert  is  1 & {\color[HTML]{9D7500} 0.206} & {\color[HTML]{59B900} 0.211} & {\color[HTML]{AA6800} 0.273} & {\color[HTML]{32E100} 0.608} & {\color[HTML]{44CE00} 0.193} & {\color[HTML]{3AD800} 0.186} & {\color[HTML]{3AD800} 0.243} & {\color[HTML]{D73B00} 0.641} & {\color[HTML]{3ED400} 0.229} & {\color[HTML]{33DF00} 0.2} & {\color[HTML]{39D900} 0.28} & {\color[HTML]{DA3800} 0.64} & {\color[HTML]{49C900} 0.25} & {\color[HTML]{36DC00} 0.18} & {\color[HTML]{43CF00} 0.28} & {\color[HTML]{DD3500} 0.692} \\
llama7 & focal  one  bert  is  1 & {\color[HTML]{E13200} 0.063} & {\color[HTML]{DA3800} 0.041} & {\color[HTML]{E13200} 0.213} & {\color[HTML]{56BC00} 0.629} & {\color[HTML]{55BD00} 0.068} & {\color[HTML]{4EC400} 0.045} & {\color[HTML]{42D000} 0.182} & {\color[HTML]{D83A00} 0.65} & {\color[HTML]{51C100} 0.083} & {\color[HTML]{46CC00} 0.074} & {\color[HTML]{40D200} 0.227} & {\color[HTML]{DA3800} 0.641} & {\color[HTML]{5EB400} 0.076} & {\color[HTML]{49C900} 0.048} & {\color[HTML]{4BC700} 0.211} & {\color[HTML]{DC3600} 0.683} \\
\hline
llama8 & LLM Prob. & {\color[HTML]{759D00} 0.294} & {\color[HTML]{7A9800} 0.137} & {\color[HTML]{9C7600} 0.281} & {\color[HTML]{E03200} 0.763} & {\color[HTML]{32E000} 0.356} & {\color[HTML]{35DD00} 0.197} & {\color[HTML]{32E000} 0.329} & {\color[HTML]{E03200} 0.742} & {\color[HTML]{32E000} 0.305} & {\color[HTML]{39D900} 0.189} & {\color[HTML]{32E000} 0.33} & {\color[HTML]{DE3400} 0.64} & {\color[HTML]{32E000} 0.274} & {\color[HTML]{46CC00} 0.065} & {\color[HTML]{32E000} 0.312} & {\color[HTML]{D24000} 0.618} \\
llama8 & LLM Prob + PS & {\color[HTML]{888A00} 0.257} & {\color[HTML]{C94900} 0.068} & {\color[HTML]{9C7600} 0.281} & {\color[HTML]{4CC600} 0.655} & {\color[HTML]{3FD300} 0.255} & {\color[HTML]{44CE00} 0.094} & {\color[HTML]{39D900} 0.27} & {\color[HTML]{E03200} 0.742} & {\color[HTML]{43CF00} 0.171} & {\color[HTML]{4DC500} 0.048} & {\color[HTML]{3AD800} 0.265} & {\color[HTML]{DE3400} 0.64} & {\color[HTML]{3DD500} 0.189} & {\color[HTML]{4AC800} 0.034} & {\color[HTML]{36DC00} 0.278} & {\color[HTML]{D24000} 0.618} \\
llama8 & verb  prob & {\color[HTML]{32E000} 0.429} & {\color[HTML]{B85A00} 0.083} & {\color[HTML]{32E000} 0.399} & {\color[HTML]{55BD00} 0.662} & {\color[HTML]{E13200}     -} & {\color[HTML]{E13200}     -} & {\color[HTML]{E13200}     -} & {\color[HTML]{32E100}     -} & {\color[HTML]{E13200}     -} & {\color[HTML]{E13200}     -} & {\color[HTML]{E13200}     -} & {\color[HTML]{32E100}     -} & {\color[HTML]{E13200}     -} & {\color[HTML]{E13200}     -} & {\color[HTML]{E13200}     -} & {\color[HTML]{32E100}     -} \\
llama8 & Calib  -(cluster) & {\color[HTML]{C15100} 0.143} & {\color[HTML]{9F7300} 0.105} & {\color[HTML]{CC4600} 0.228} & {\color[HTML]{3DD500} 0.644} & {\color[HTML]{50C200} 0.12} & {\color[HTML]{40D200} 0.118} & {\color[HTML]{40D200} 0.218} & {\color[HTML]{D73B00} 0.646} & {\color[HTML]{48CA00} 0.14} & {\color[HTML]{42D000} 0.127} & {\color[HTML]{3CD600} 0.249} & {\color[HTML]{DE3400} 0.634} & {\color[HTML]{47CB00} 0.121} & {\color[HTML]{44CE00} 0.076} & {\color[HTML]{3DD500} 0.227} & {\color[HTML]{DB3700} 0.703} \\
llama8 & Calib  - & {\color[HTML]{D53D00} 0.103} & {\color[HTML]{BD5500} 0.079} & {\color[HTML]{DC3600} 0.21} & {\color[HTML]{54BE00} 0.661} & {\color[HTML]{52C000} 0.102} & {\color[HTML]{46CC00} 0.076} & {\color[HTML]{41D100} 0.214} & {\color[HTML]{D63C00} 0.639} & {\color[HTML]{52C000} 0.066} & {\color[HTML]{4CC600} 0.054} & {\color[HTML]{3ED400} 0.237} & {\color[HTML]{DC3600} 0.619} & {\color[HTML]{48CA00} 0.111} & {\color[HTML]{43CF00} 0.085} & {\color[HTML]{3ED400} 0.215} & {\color[HTML]{DD3500} 0.73} \\
llama8 & Calib-7 & {\color[HTML]{D14100} 0.112} & {\color[HTML]{C54D00} 0.072} & {\color[HTML]{DF3300} 0.207} & {\color[HTML]{809200} 0.693} & {\color[HTML]{52C000} 0.108} & {\color[HTML]{45CD00} 0.083} & {\color[HTML]{41D100} 0.214} & {\color[HTML]{D83A00} 0.655} & {\color[HTML]{4EC400} 0.091} & {\color[HTML]{49C900} 0.076} & {\color[HTML]{3ED400} 0.232} & {\color[HTML]{E03200} 0.66} & {\color[HTML]{4CC600} 0.084} & {\color[HTML]{45CD00} 0.072} & {\color[HTML]{40D200} 0.205} & {\color[HTML]{DF3300} 0.747} \\
llama8 & Calib-5 + PS & {\color[HTML]{B65C00} 0.166} & {\color[HTML]{E13200} 0.048} & {\color[HTML]{C54D00} 0.236} & {\color[HTML]{32E100} 0.636} & {\color[HTML]{4AC800} 0.166} & {\color[HTML]{4BC700} 0.044} & {\color[HTML]{3ED400} 0.236} & {\color[HTML]{D83A00} 0.655} & {\color[HTML]{4BC700} 0.117} & {\color[HTML]{4BC700} 0.063} & {\color[HTML]{3DD500} 0.242} & {\color[HTML]{E03200} 0.66} & {\color[HTML]{45CD00} 0.133} & {\color[HTML]{3ED400} 0.121} & {\color[HTML]{3CD600} 0.231} & {\color[HTML]{DF3300} 0.747} \\
llama8 & bce-auc  small  bert  is  7 & {\color[HTML]{D14100} 0.112} & {\color[HTML]{C54D00} 0.072} & {\color[HTML]{DF3300} 0.207} & {\color[HTML]{809200} 0.693} & {\color[HTML]{52C000} 0.108} & {\color[HTML]{45CD00} 0.084} & {\color[HTML]{41D100} 0.214} & {\color[HTML]{D83A00} 0.654} & {\color[HTML]{4FC300} 0.088} & {\color[HTML]{49C900} 0.077} & {\color[HTML]{3ED400} 0.232} & {\color[HTML]{E03200} 0.66} & {\color[HTML]{4CC600} 0.083} & {\color[HTML]{45CD00} 0.071} & {\color[HTML]{40D200} 0.205} & {\color[HTML]{DF3300} 0.747} \\
llama8 & (auc)Calib-7 & {\color[HTML]{A27000} 0.205} & {\color[HTML]{3AD800} 0.193} & {\color[HTML]{B26000} 0.256} & {\color[HTML]{7C9600} 0.69} & {\color[HTML]{42D000} 0.227} & {\color[HTML]{32E000} 0.222} & {\color[HTML]{38DA00} 0.279} & {\color[HTML]{D73B00} 0.648} & {\color[HTML]{3AD800} 0.244} & {\color[HTML]{32E000} 0.242} & {\color[HTML]{36DC00} 0.297} & {\color[HTML]{DD3500} 0.631} & {\color[HTML]{39D900} 0.217} & {\color[HTML]{32E000} 0.204} & {\color[HTML]{3AD800} 0.249} & {\color[HTML]{E03200} 0.763} \\
llama8 & (focal)Calib-7 & {\color[HTML]{CB4700} 0.123} & {\color[HTML]{AE6400} 0.092} & {\color[HTML]{CF4300} 0.224} & {\color[HTML]{37DB00} 0.64} & {\color[HTML]{54BE00} 0.092} & {\color[HTML]{46CC00} 0.078} & {\color[HTML]{41D100} 0.211} & {\color[HTML]{D83A00} 0.658} & {\color[HTML]{50C200} 0.078} & {\color[HTML]{4BC700} 0.058} & {\color[HTML]{3FD300} 0.229} & {\color[HTML]{E03200} 0.659} & {\color[HTML]{4DC500} 0.074} & {\color[HTML]{46CC00} 0.062} & {\color[HTML]{40D200} 0.204} & {\color[HTML]{DF3300} 0.749} \\
llama8 & auc  one  bert  is  1 & {\color[HTML]{A46E00} 0.201} & {\color[HTML]{32E000} 0.2} & {\color[HTML]{B06200} 0.259} & {\color[HTML]{50C200} 0.658} & {\color[HTML]{46CC00} 0.197} & {\color[HTML]{37DB00} 0.186} & {\color[HTML]{3BD700} 0.254} & {\color[HTML]{D43E00} 0.619} & {\color[HTML]{3CD600} 0.224} & {\color[HTML]{3CD600} 0.168} & {\color[HTML]{38DA00} 0.284} & {\color[HTML]{DD3500} 0.627} & {\color[HTML]{3AD800} 0.215} & {\color[HTML]{38DA00} 0.161} & {\color[HTML]{39D900} 0.258} & {\color[HTML]{DD3500} 0.73} \\
llama8 & focal  one  bert  is  1 & {\color[HTML]{E13200} 0.081} & {\color[HTML]{C74B00} 0.07} & {\color[HTML]{E13200} 0.205} & {\color[HTML]{58BA00} 0.664} & {\color[HTML]{54BE00} 0.087} & {\color[HTML]{46CC00} 0.077} & {\color[HTML]{41D100} 0.213} & {\color[HTML]{D43E00} 0.616} & {\color[HTML]{53BF00} 0.056} & {\color[HTML]{4DC500} 0.048} & {\color[HTML]{3ED400} 0.235} & {\color[HTML]{DC3600} 0.616} & {\color[HTML]{4BC700} 0.09} & {\color[HTML]{45CD00} 0.072} & {\color[HTML]{3ED400} 0.215} & {\color[HTML]{DB3700} 0.71} \\
\hline
llama31-8 & LLM Prob. & {\color[HTML]{947E00} 0.26} & {\color[HTML]{8A8800} 0.114} & {\color[HTML]{B85A00} 0.244} & {\color[HTML]{E03200} 0.786} & {\color[HTML]{38DA00} 0.183} & {\color[HTML]{3FD300} 0.123} & {\color[HTML]{35DD00} 0.247} & {\color[HTML]{DB3700} 0.718} & {\color[HTML]{32E000} 0.316} & {\color[HTML]{3AD800} 0.163} & {\color[HTML]{32E000} 0.333} & {\color[HTML]{D63C00} 0.651} & {\color[HTML]{3BD700} 0.16} & {\color[HTML]{49C900} 0.048} & {\color[HTML]{33DF00} 0.242} & {\color[HTML]{DB3700} 0.693} \\
llama31-8 & LLM Prob + PS & {\color[HTML]{878B00} 0.295} & {\color[HTML]{CC4600} 0.054} & {\color[HTML]{9F7300} 0.287} & {\color[HTML]{32E100} 0.614} & {\color[HTML]{32E000} 0.231} & {\color[HTML]{41D100} 0.109} & {\color[HTML]{34DE00} 0.25} & {\color[HTML]{E03200} 0.773} & {\color[HTML]{3DD500} 0.226} & {\color[HTML]{4AC800} 0.052} & {\color[HTML]{38DA00} 0.281} & {\color[HTML]{D63C00} 0.651} & {\color[HTML]{39D900} 0.177} & {\color[HTML]{48CA00} 0.059} & {\color[HTML]{32E000} 0.256} & {\color[HTML]{DB3700} 0.694} \\
llama31-8 & verb  prob & {\color[HTML]{32E000} 0.52} & {\color[HTML]{59B900} 0.159} & {\color[HTML]{32E000} 0.48} & {\color[HTML]{4AC800} 0.638} & {\color[HTML]{E13200}     -} & {\color[HTML]{E13200}     -} & {\color[HTML]{E13200}     -} & {\color[HTML]{32E100}     -} & {\color[HTML]{E13200}     -} & {\color[HTML]{E13200}     -} & {\color[HTML]{E13200}     -} & {\color[HTML]{32E100}     -} & {\color[HTML]{E13200}     -} & {\color[HTML]{E13200}     -} & {\color[HTML]{E13200}     -} & {\color[HTML]{32E100}     -} \\
llama31-8 & Calib  -(cluster) & {\color[HTML]{C74B00} 0.126} & {\color[HTML]{947E00} 0.105} & {\color[HTML]{CF4300} 0.202} & {\color[HTML]{63AF00} 0.663} & {\color[HTML]{42D000} 0.114} & {\color[HTML]{46CC00} 0.077} & {\color[HTML]{3AD800} 0.209} & {\color[HTML]{DA3800} 0.706} & {\color[HTML]{4EC400} 0.1} & {\color[HTML]{47CB00} 0.072} & {\color[HTML]{41D100} 0.215} & {\color[HTML]{DD3500} 0.718} & {\color[HTML]{42D000} 0.111} & {\color[HTML]{46CC00} 0.071} & {\color[HTML]{36DC00} 0.223} & {\color[HTML]{DC3600} 0.706} \\
llama31-8 & Calib  - & {\color[HTML]{DB3700} 0.073} & {\color[HTML]{B95900} 0.071} & {\color[HTML]{E03200} 0.173} & {\color[HTML]{A76B00} 0.729} & {\color[HTML]{44CE00} 0.101} & {\color[HTML]{43CF00} 0.095} & {\color[HTML]{3AD800} 0.207} & {\color[HTML]{D93900} 0.699} & {\color[HTML]{51C100} 0.081} & {\color[HTML]{49C900} 0.062} & {\color[HTML]{44CE00} 0.195} & {\color[HTML]{E03200} 0.754} & {\color[HTML]{45CD00} 0.09} & {\color[HTML]{47CB00} 0.067} & {\color[HTML]{38DA00} 0.21} & {\color[HTML]{DD3500} 0.714} \\
llama31-8 & Calib-7 & {\color[HTML]{D73B00} 0.085} & {\color[HTML]{BB5700} 0.069} & {\color[HTML]{DF3300} 0.175} & {\color[HTML]{AC6600} 0.734} & {\color[HTML]{44CE00} 0.101} & {\color[HTML]{48CA00} 0.063} & {\color[HTML]{3BD700} 0.203} & {\color[HTML]{DB3700} 0.714} & {\color[HTML]{51C100} 0.078} & {\color[HTML]{4AC800} 0.05} & {\color[HTML]{43CF00} 0.199} & {\color[HTML]{E03200} 0.747} & {\color[HTML]{48CA00} 0.072} & {\color[HTML]{48CA00} 0.055} & {\color[HTML]{39D900} 0.201} & {\color[HTML]{E03200} 0.743} \\
llama31-8 & Calib-5 + PS & {\color[HTML]{A66C00} 0.214} & {\color[HTML]{E13200} 0.035} & {\color[HTML]{BD5500} 0.234} & {\color[HTML]{48CA00} 0.636} & {\color[HTML]{3AD800} 0.173} & {\color[HTML]{45CD00} 0.081} & {\color[HTML]{36DC00} 0.236} & {\color[HTML]{DB3700} 0.714} & {\color[HTML]{47CB00} 0.156} & {\color[HTML]{41D100} 0.118} & {\color[HTML]{3ED400} 0.239} & {\color[HTML]{E03200} 0.747} & {\color[HTML]{41D100} 0.124} & {\color[HTML]{3ED400} 0.128} & {\color[HTML]{36DC00} 0.227} & {\color[HTML]{E03200} 0.743} \\
llama31-8 & bce-auc  small  bert  is  7 & {\color[HTML]{D73B00} 0.085} & {\color[HTML]{BB5700} 0.069} & {\color[HTML]{DF3300} 0.175} & {\color[HTML]{AC6600} 0.734} & {\color[HTML]{44CE00} 0.1} & {\color[HTML]{48CA00} 0.062} & {\color[HTML]{3BD700} 0.203} & {\color[HTML]{DB3700} 0.713} & {\color[HTML]{51C100} 0.079} & {\color[HTML]{4AC800} 0.051} & {\color[HTML]{43CF00} 0.199} & {\color[HTML]{E03200} 0.746} & {\color[HTML]{48CA00} 0.072} & {\color[HTML]{48CA00} 0.056} & {\color[HTML]{39D900} 0.201} & {\color[HTML]{E03200} 0.743} \\
llama31-8 & (auc)Calib-7 & {\color[HTML]{A86A00} 0.209} & {\color[HTML]{32E000} 0.195} & {\color[HTML]{BA5800} 0.239} & {\color[HTML]{A56D00} 0.728} & {\color[HTML]{35DD00} 0.207} & {\color[HTML]{33DF00} 0.203} & {\color[HTML]{33DF00} 0.262} & {\color[HTML]{DA3800} 0.704} & {\color[HTML]{3BD700} 0.246} & {\color[HTML]{32E000} 0.223} & {\color[HTML]{38DA00} 0.282} & {\color[HTML]{D93900} 0.679} & {\color[HTML]{32E000} 0.23} & {\color[HTML]{32E000} 0.214} & {\color[HTML]{32E000} 0.251} & {\color[HTML]{E03200} 0.753} \\
llama31-8 & (focal)Calib-7 & {\color[HTML]{CB4700} 0.116} & {\color[HTML]{928000} 0.107} & {\color[HTML]{CE4400} 0.205} & {\color[HTML]{45CD00} 0.633} & {\color[HTML]{45CD00} 0.092} & {\color[HTML]{47CB00} 0.068} & {\color[HTML]{3BD700} 0.201} & {\color[HTML]{DA3800} 0.709} & {\color[HTML]{50C200} 0.088} & {\color[HTML]{49C900} 0.056} & {\color[HTML]{43CF00} 0.199} & {\color[HTML]{DF3300} 0.742} & {\color[HTML]{48CA00} 0.07} & {\color[HTML]{49C900} 0.051} & {\color[HTML]{39D900} 0.201} & {\color[HTML]{DF3300} 0.742} \\
llama31-8 & auc  one  bert  is  1 & {\color[HTML]{A36F00} 0.22} & {\color[HTML]{32E000} 0.195} & {\color[HTML]{B55D00} 0.249} & {\color[HTML]{8F8300} 0.706} & {\color[HTML]{32E000} 0.231} & {\color[HTML]{32E000} 0.216} & {\color[HTML]{32E000} 0.27} & {\color[HTML]{D83A00} 0.685} & {\color[HTML]{35DD00} 0.292} & {\color[HTML]{38DA00} 0.177} & {\color[HTML]{37DB00} 0.292} & {\color[HTML]{DF3300} 0.734} & {\color[HTML]{40D200} 0.127} & {\color[HTML]{3DD500} 0.136} & {\color[HTML]{36DC00} 0.221} & {\color[HTML]{DD3500} 0.716} \\
llama31-8 & focal  one  bert  is  1 & {\color[HTML]{E13200} 0.059} & {\color[HTML]{C15100} 0.064} & {\color[HTML]{E13200} 0.172} & {\color[HTML]{A27000} 0.725} & {\color[HTML]{48CA00} 0.071} & {\color[HTML]{46CC00} 0.072} & {\color[HTML]{3BD700} 0.201} & {\color[HTML]{D93900} 0.694} & {\color[HTML]{53BF00} 0.065} & {\color[HTML]{4AC800} 0.052} & {\color[HTML]{44CE00} 0.194} & {\color[HTML]{E03200} 0.747} & {\color[HTML]{49C900} 0.067} & {\color[HTML]{4AC800} 0.045} & {\color[HTML]{39D900} 0.205} & {\color[HTML]{DD3500} 0.716} \\
\hline
gemma2 & LLM Prob. & {\color[HTML]{AF6300} 0.182} & {\color[HTML]{A27000} 0.098} & {\color[HTML]{D43E00} 0.209} & {\color[HTML]{E03200} 0.776} & {\color[HTML]{3BD700} 0.191} & {\color[HTML]{46CC00} 0.1} & {\color[HTML]{3DD500} 0.211} & {\color[HTML]{E03200} 0.798} & {\color[HTML]{3ED400} 0.173} & {\color[HTML]{42D000} 0.124} & {\color[HTML]{3AD800} 0.245} & {\color[HTML]{E03200} 0.703} & {\color[HTML]{41D100} 0.174} & {\color[HTML]{42D000} 0.148} & {\color[HTML]{38DA00} 0.261} & {\color[HTML]{D83A00} 0.641} \\
gemma2 & LLM Prob + PS & {\color[HTML]{8C8600} 0.285} & {\color[HTML]{E13200} 0.016} & {\color[HTML]{AF6300} 0.277} & {\color[HTML]{32E100} 0.638} & {\color[HTML]{32E000} 0.261} & {\color[HTML]{44CE00} 0.116} & {\color[HTML]{37DB00} 0.25} & {\color[HTML]{E03200} 0.798} & {\color[HTML]{3AD800} 0.203} & {\color[HTML]{4AC800} 0.069} & {\color[HTML]{39D900} 0.254} & {\color[HTML]{E03200} 0.703} & {\color[HTML]{41D100} 0.176} & {\color[HTML]{51C100} 0.035} & {\color[HTML]{39D900} 0.254} & {\color[HTML]{D83A00} 0.641} \\
gemma2 & verb  prob & {\color[HTML]{32E000} 0.55} & {\color[HTML]{967C00} 0.115} & {\color[HTML]{32E000} 0.509} & {\color[HTML]{47CB00} 0.655} & {\color[HTML]{E13200}     -} & {\color[HTML]{E13200}     -} & {\color[HTML]{E13200}     -} & {\color[HTML]{32E100}     -} & {\color[HTML]{E13200}     -} & {\color[HTML]{E13200}     -} & {\color[HTML]{E13200}     -} & {\color[HTML]{32E100}     -} & {\color[HTML]{E13200}     -} & {\color[HTML]{E13200}     -} & {\color[HTML]{E13200}     -} & {\color[HTML]{32E100}     -} \\
gemma2 & Calib  -(cluster) & {\color[HTML]{C05200} 0.132} & {\color[HTML]{A96900} 0.089} & {\color[HTML]{D63C00} 0.205} & {\color[HTML]{51C100} 0.663} & {\color[HTML]{45CD00} 0.122} & {\color[HTML]{44CE00} 0.111} & {\color[HTML]{3DD500} 0.211} & {\color[HTML]{D33F00} 0.661} & {\color[HTML]{42D000} 0.144} & {\color[HTML]{45CD00} 0.108} & {\color[HTML]{3CD600} 0.232} & {\color[HTML]{DA3800} 0.641} & {\color[HTML]{49C900} 0.115} & {\color[HTML]{4BC700} 0.078} & {\color[HTML]{3DD500} 0.218} & {\color[HTML]{DE3400} 0.702} \\
gemma2 & Calib  - & {\color[HTML]{D24000} 0.08} & {\color[HTML]{C44E00} 0.054} & {\color[HTML]{DC3600} 0.193} & {\color[HTML]{35DD00} 0.641} & {\color[HTML]{48CA00} 0.096} & {\color[HTML]{4AC800} 0.075} & {\color[HTML]{3ED400} 0.205} & {\color[HTML]{D24000} 0.644} & {\color[HTML]{4AC800} 0.085} & {\color[HTML]{4DC500} 0.048} & {\color[HTML]{3ED400} 0.216} & {\color[HTML]{D93900} 0.633} & {\color[HTML]{4BC700} 0.102} & {\color[HTML]{4CC600} 0.077} & {\color[HTML]{3ED400} 0.212} & {\color[HTML]{DE3400} 0.706} \\
gemma2 & Calib-7 & {\color[HTML]{CD4500} 0.093} & {\color[HTML]{AD6500} 0.084} & {\color[HTML]{DD3500} 0.191} & {\color[HTML]{55BD00} 0.666} & {\color[HTML]{48CA00} 0.098} & {\color[HTML]{48CA00} 0.088} & {\color[HTML]{3DD500} 0.206} & {\color[HTML]{D33F00} 0.664} & {\color[HTML]{4BC700} 0.082} & {\color[HTML]{48CA00} 0.08} & {\color[HTML]{3ED400} 0.214} & {\color[HTML]{DC3600} 0.661} & {\color[HTML]{4BC700} 0.099} & {\color[HTML]{4BC700} 0.085} & {\color[HTML]{3ED400} 0.212} & {\color[HTML]{E03200} 0.72} \\
gemma2 & Calib-5 + PS & {\color[HTML]{A46E00} 0.213} & {\color[HTML]{D73B00} 0.028} & {\color[HTML]{C44E00} 0.237} & {\color[HTML]{41D100} 0.65} & {\color[HTML]{39D900} 0.205} & {\color[HTML]{4EC400} 0.043} & {\color[HTML]{39D900} 0.241} & {\color[HTML]{D33F00} 0.664} & {\color[HTML]{3DD500} 0.178} & {\color[HTML]{4CC600} 0.057} & {\color[HTML]{3AD800} 0.248} & {\color[HTML]{DC3600} 0.661} & {\color[HTML]{41D100} 0.173} & {\color[HTML]{49C900} 0.093} & {\color[HTML]{3AD800} 0.244} & {\color[HTML]{E03200} 0.72} \\
gemma2 & bce-auc  small  bert  is  7 & {\color[HTML]{CD4500} 0.093} & {\color[HTML]{AD6500} 0.084} & {\color[HTML]{DD3500} 0.191} & {\color[HTML]{55BD00} 0.666} & {\color[HTML]{48CA00} 0.098} & {\color[HTML]{48CA00} 0.087} & {\color[HTML]{3DD500} 0.206} & {\color[HTML]{D33F00} 0.664} & {\color[HTML]{4BC700} 0.08} & {\color[HTML]{49C900} 0.076} & {\color[HTML]{3ED400} 0.213} & {\color[HTML]{DC3600} 0.662} & {\color[HTML]{4BC700} 0.098} & {\color[HTML]{4BC700} 0.085} & {\color[HTML]{3ED400} 0.212} & {\color[HTML]{E03200} 0.72} \\
gemma2 & (auc)Calib-7 & {\color[HTML]{957D00} 0.259} & {\color[HTML]{32E000} 0.247} & {\color[HTML]{A76B00} 0.292} & {\color[HTML]{46CC00} 0.654} & {\color[HTML]{32E000} 0.26} & {\color[HTML]{32E000} 0.246} & {\color[HTML]{32E000} 0.294} & {\color[HTML]{D24000} 0.651} & {\color[HTML]{32E000} 0.263} & {\color[HTML]{32E000} 0.243} & {\color[HTML]{32E000} 0.308} & {\color[HTML]{DA3800} 0.641} & {\color[HTML]{32E000} 0.288} & {\color[HTML]{32E000} 0.266} & {\color[HTML]{32E000} 0.307} & {\color[HTML]{E03200} 0.726} \\
gemma2 & (focal)Calib-7 & {\color[HTML]{CD4500} 0.095} & {\color[HTML]{B06200} 0.08} & {\color[HTML]{DB3700} 0.196} & {\color[HTML]{46CC00} 0.654} & {\color[HTML]{49C900} 0.095} & {\color[HTML]{48CA00} 0.087} & {\color[HTML]{3ED400} 0.205} & {\color[HTML]{D33F00} 0.659} & {\color[HTML]{4DC500} 0.066} & {\color[HTML]{4BC700} 0.06} & {\color[HTML]{3FD300} 0.21} & {\color[HTML]{DC3600} 0.664} & {\color[HTML]{4BC700} 0.098} & {\color[HTML]{4BC700} 0.081} & {\color[HTML]{3ED400} 0.211} & {\color[HTML]{E03200} 0.717} \\
gemma2 & auc  one  bert  is  1 & {\color[HTML]{A17100} 0.224} & {\color[HTML]{6FA300} 0.166} & {\color[HTML]{BA5800} 0.257} & {\color[HTML]{3DD500} 0.647} & {\color[HTML]{35DD00} 0.237} & {\color[HTML]{3DD500} 0.162} & {\color[HTML]{35DD00} 0.269} & {\color[HTML]{D24000} 0.65} & {\color[HTML]{3BD700} 0.196} & {\color[HTML]{3CD600} 0.167} & {\color[HTML]{37DB00} 0.269} & {\color[HTML]{D93900} 0.631} & {\color[HTML]{38DA00} 0.241} & {\color[HTML]{3CD600} 0.193} & {\color[HTML]{36DC00} 0.273} & {\color[HTML]{DF3300} 0.716} \\
gemma2 & focal  one  bert  is  1 & {\color[HTML]{E13200} 0.037} & {\color[HTML]{D43E00} 0.032} & {\color[HTML]{E13200} 0.185} & {\color[HTML]{3CD600} 0.646} & {\color[HTML]{4BC700} 0.074} & {\color[HTML]{4CC600} 0.06} & {\color[HTML]{3ED400} 0.202} & {\color[HTML]{D24000} 0.645} & {\color[HTML]{4FC300} 0.052} & {\color[HTML]{4EC400} 0.044} & {\color[HTML]{3ED400} 0.212} & {\color[HTML]{DA3800} 0.636} & {\color[HTML]{4EC400} 0.078} & {\color[HTML]{4DC500} 0.065} & {\color[HTML]{3ED400} 0.21} & {\color[HTML]{DE3400} 0.7} \\
\hline
gemma9 & LLM Prob. & {\color[HTML]{819100} 0.278} & {\color[HTML]{34DE00} 0.195} & {\color[HTML]{A07200} 0.296} & {\color[HTML]{E03200} 0.723} & {\color[HTML]{32E000} 0.293} & {\color[HTML]{37DB00} 0.179} & {\color[HTML]{32E000} 0.293} & {\color[HTML]{E03200} 0.757} & {\color[HTML]{32E000} 0.251} & {\color[HTML]{39D900} 0.175} & {\color[HTML]{32E000} 0.291} & {\color[HTML]{E03200} 0.668} & {\color[HTML]{38DA00} 0.187} & {\color[HTML]{3BD700} 0.161} & {\color[HTML]{32E000} 0.266} & {\color[HTML]{D53D00} 0.604} \\
gemma9 & LLM Prob + PS & {\color[HTML]{B35F00} 0.177} & {\color[HTML]{E13200} 0.045} & {\color[HTML]{C25000} 0.26} & {\color[HTML]{BA5800} 0.697} & {\color[HTML]{3DD500} 0.206} & {\color[HTML]{42D000} 0.102} & {\color[HTML]{37DB00} 0.254} & {\color[HTML]{E03200} 0.757} & {\color[HTML]{41D100} 0.137} & {\color[HTML]{49C900} 0.065} & {\color[HTML]{38DA00} 0.246} & {\color[HTML]{E03200} 0.669} & {\color[HTML]{44CE00} 0.107} & {\color[HTML]{4EC400} 0.034} & {\color[HTML]{36DC00} 0.236} & {\color[HTML]{D53D00} 0.604} \\
gemma9 & verb  prob & {\color[HTML]{32E000} 0.438} & {\color[HTML]{72A000} 0.141} & {\color[HTML]{32E000} 0.414} & {\color[HTML]{C64C00} 0.705} & {\color[HTML]{E13200}     -} & {\color[HTML]{E13200}     -} & {\color[HTML]{E13200}     -} & {\color[HTML]{32E100}     -} & {\color[HTML]{E13200}     -} & {\color[HTML]{E13200}     -} & {\color[HTML]{E13200}     -} & {\color[HTML]{32E100}     -} & {\color[HTML]{E13200}     -} & {\color[HTML]{E13200}     -} & {\color[HTML]{E13200}     -} & {\color[HTML]{32E100}     -} \\
gemma9 & Calib  -(cluster) & {\color[HTML]{C05200} 0.151} & {\color[HTML]{967C00} 0.11} & {\color[HTML]{D24000} 0.242} & {\color[HTML]{68AA00} 0.641} & {\color[HTML]{48CA00} 0.13} & {\color[HTML]{42D000} 0.102} & {\color[HTML]{39D900} 0.235} & {\color[HTML]{D63C00} 0.647} & {\color[HTML]{3FD300} 0.153} & {\color[HTML]{40D200} 0.124} & {\color[HTML]{36DC00} 0.255} & {\color[HTML]{DD3500} 0.632} & {\color[HTML]{42D000} 0.121} & {\color[HTML]{44CE00} 0.098} & {\color[HTML]{37DB00} 0.225} & {\color[HTML]{DC3600} 0.674} \\
gemma9 & Calib  - & {\color[HTML]{D04200} 0.12} & {\color[HTML]{C05200} 0.073} & {\color[HTML]{DC3600} 0.232} & {\color[HTML]{45CD00} 0.617} & {\color[HTML]{4DC500} 0.089} & {\color[HTML]{48CA00} 0.058} & {\color[HTML]{3AD800} 0.227} & {\color[HTML]{D33F00} 0.626} & {\color[HTML]{4AC800} 0.079} & {\color[HTML]{4BC700} 0.048} & {\color[HTML]{39D900} 0.234} & {\color[HTML]{DB3700} 0.618} & {\color[HTML]{45CD00} 0.098} & {\color[HTML]{45CD00} 0.091} & {\color[HTML]{39D900} 0.211} & {\color[HTML]{DE3400} 0.694} \\
gemma9 & Calib-7 & {\color[HTML]{BD5500} 0.158} & {\color[HTML]{BC5600} 0.077} & {\color[HTML]{CE4400} 0.247} & {\color[HTML]{71A100} 0.647} & {\color[HTML]{46CC00} 0.139} & {\color[HTML]{46CC00} 0.072} & {\color[HTML]{39D900} 0.238} & {\color[HTML]{D63C00} 0.653} & {\color[HTML]{46CC00} 0.106} & {\color[HTML]{49C900} 0.066} & {\color[HTML]{39D900} 0.235} & {\color[HTML]{DE3400} 0.642} & {\color[HTML]{47CB00} 0.082} & {\color[HTML]{48CA00} 0.074} & {\color[HTML]{3AD800} 0.206} & {\color[HTML]{E03200} 0.711} \\
gemma9 & Calib-5 + PS & {\color[HTML]{D83A00} 0.104} & {\color[HTML]{DD3500} 0.048} & {\color[HTML]{DF3300} 0.229} & {\color[HTML]{68AA00} 0.641} & {\color[HTML]{4CC600} 0.096} & {\color[HTML]{4CC600} 0.032} & {\color[HTML]{3AD800} 0.231} & {\color[HTML]{D63C00} 0.653} & {\color[HTML]{49C900} 0.082} & {\color[HTML]{4BC700} 0.05} & {\color[HTML]{39D900} 0.233} & {\color[HTML]{DE3400} 0.642} & {\color[HTML]{46CC00} 0.091} & {\color[HTML]{47CB00} 0.081} & {\color[HTML]{38DA00} 0.219} & {\color[HTML]{E03200} 0.711} \\
gemma9 & bce-auc  small  bert  is  7 & {\color[HTML]{BD5500} 0.158} & {\color[HTML]{BC5600} 0.077} & {\color[HTML]{CE4400} 0.247} & {\color[HTML]{71A100} 0.647} & {\color[HTML]{46CC00} 0.138} & {\color[HTML]{46CC00} 0.071} & {\color[HTML]{39D900} 0.237} & {\color[HTML]{D63C00} 0.653} & {\color[HTML]{46CC00} 0.105} & {\color[HTML]{48CA00} 0.068} & {\color[HTML]{39D900} 0.236} & {\color[HTML]{DE3400} 0.641} & {\color[HTML]{47CB00} 0.081} & {\color[HTML]{48CA00} 0.074} & {\color[HTML]{3AD800} 0.206} & {\color[HTML]{E03200} 0.711} \\
gemma9 & (auc)Calib-7 & {\color[HTML]{9A7800} 0.227} & {\color[HTML]{32E000} 0.197} & {\color[HTML]{AD6500} 0.282} & {\color[HTML]{65AD00} 0.639} & {\color[HTML]{39D900} 0.237} & {\color[HTML]{32E000} 0.217} & {\color[HTML]{32E000} 0.287} & {\color[HTML]{D53D00} 0.645} & {\color[HTML]{35DD00} 0.227} & {\color[HTML]{32E000} 0.229} & {\color[HTML]{32E000} 0.286} & {\color[HTML]{DB3700} 0.619} & {\color[HTML]{32E000} 0.236} & {\color[HTML]{32E000} 0.231} & {\color[HTML]{32E000} 0.26} & {\color[HTML]{E03200} 0.714} \\
gemma9 & (focal)Calib-7 & {\color[HTML]{BF5300} 0.154} & {\color[HTML]{BB5700} 0.078} & {\color[HTML]{CE4400} 0.247} & {\color[HTML]{63AF00} 0.638} & {\color[HTML]{49C900} 0.12} & {\color[HTML]{46CC00} 0.075} & {\color[HTML]{39D900} 0.234} & {\color[HTML]{D63C00} 0.653} & {\color[HTML]{47CB00} 0.099} & {\color[HTML]{4BC700} 0.049} & {\color[HTML]{39D900} 0.234} & {\color[HTML]{DD3500} 0.64} & {\color[HTML]{47CB00} 0.083} & {\color[HTML]{48CA00} 0.073} & {\color[HTML]{3AD800} 0.207} & {\color[HTML]{E03200} 0.709} \\
gemma9 & auc  one  bert  is  1 & {\color[HTML]{B35F00} 0.177} & {\color[HTML]{51C100} 0.17} & {\color[HTML]{B95900} 0.269} & {\color[HTML]{32E100} 0.604} & {\color[HTML]{41D100} 0.177} & {\color[HTML]{39D900} 0.168} & {\color[HTML]{36DC00} 0.262} & {\color[HTML]{D43E00} 0.632} & {\color[HTML]{39D900} 0.197} & {\color[HTML]{37DB00} 0.189} & {\color[HTML]{34DE00} 0.276} & {\color[HTML]{DA3800} 0.606} & {\color[HTML]{37DB00} 0.196} & {\color[HTML]{39D900} 0.178} & {\color[HTML]{33DF00} 0.252} & {\color[HTML]{DE3400} 0.693} \\
gemma9 & focal  one  bert  is  1 & {\color[HTML]{E13200} 0.086} & {\color[HTML]{C84A00} 0.066} & {\color[HTML]{E13200} 0.227} & {\color[HTML]{49C900} 0.62} & {\color[HTML]{4FC300} 0.075} & {\color[HTML]{48CA00} 0.059} & {\color[HTML]{3BD700} 0.225} & {\color[HTML]{D33F00} 0.623} & {\color[HTML]{4CC600} 0.062} & {\color[HTML]{4DC500} 0.039} & {\color[HTML]{39D900} 0.232} & {\color[HTML]{DB3700} 0.62} & {\color[HTML]{46CC00} 0.092} & {\color[HTML]{48CA00} 0.071} & {\color[HTML]{39D900} 0.209} & {\color[HTML]{DE3400} 0.694} \\
\hline
phi4 & LLM Prob. & {\color[HTML]{6CA600} 0.34} & {\color[HTML]{71A100} 0.148} & {\color[HTML]{8A8800} 0.303} & {\color[HTML]{DB3700} 0.79} & {\color[HTML]{32E000} 0.297} & {\color[HTML]{42D000} 0.131} & {\color[HTML]{36DC00} 0.273} & {\color[HTML]{E03200} 0.786} & {\color[HTML]{32E000} 0.259} & {\color[HTML]{3CD600} 0.129} & {\color[HTML]{33DF00} 0.269} & {\color[HTML]{E03200} 0.742} & {\color[HTML]{3DD500} 0.165} & {\color[HTML]{48CA00} 0.043} & {\color[HTML]{36DC00} 0.236} & {\color[HTML]{D93900} 0.669} \\
phi4 & LLM Prob + PS & {\color[HTML]{848E00} 0.282} & {\color[HTML]{DB3700} 0.053} & {\color[HTML]{A96900} 0.256} & {\color[HTML]{E03200} 0.793} & {\color[HTML]{39D900} 0.244} & {\color[HTML]{44CE00} 0.123} & {\color[HTML]{38DA00} 0.26} & {\color[HTML]{E03200} 0.786} & {\color[HTML]{37DB00} 0.216} & {\color[HTML]{43CF00} 0.086} & {\color[HTML]{34DE00} 0.259} & {\color[HTML]{E03200} 0.742} & {\color[HTML]{37DB00} 0.209} & {\color[HTML]{45CD00} 0.064} & {\color[HTML]{32E000} 0.271} & {\color[HTML]{D93900} 0.669} \\
phi4 & verb  prob & {\color[HTML]{32E000} 0.483} & {\color[HTML]{CC4600} 0.066} & {\color[HTML]{32E000} 0.439} & {\color[HTML]{7B9700} 0.739} & {\color[HTML]{E13200}     -} & {\color[HTML]{E13200}     -} & {\color[HTML]{E13200}     -} & {\color[HTML]{32E100}     -} & {\color[HTML]{E13200}     -} & {\color[HTML]{E13200}     -} & {\color[HTML]{E13200}     -} & {\color[HTML]{32E100}     -} & {\color[HTML]{E13200}     -} & {\color[HTML]{E13200}     -} & {\color[HTML]{E13200}     -} & {\color[HTML]{32E100}     -} \\
phi4 & Calib  -(cluster) & {\color[HTML]{CE4400} 0.102} & {\color[HTML]{CE4400} 0.065} & {\color[HTML]{D83A00} 0.184} & {\color[HTML]{42D000} 0.709} & {\color[HTML]{4AC800} 0.119} & {\color[HTML]{48CA00} 0.09} & {\color[HTML]{3ED400} 0.211} & {\color[HTML]{D83A00} 0.704} & {\color[HTML]{45CD00} 0.121} & {\color[HTML]{3FD300} 0.111} & {\color[HTML]{38DA00} 0.227} & {\color[HTML]{D83A00} 0.661} & {\color[HTML]{44CE00} 0.115} & {\color[HTML]{45CD00} 0.067} & {\color[HTML]{39D900} 0.214} & {\color[HTML]{DB3700} 0.686} \\
phi4 & Calib  - & {\color[HTML]{D43E00} 0.087} & {\color[HTML]{CA4800} 0.068} & {\color[HTML]{DD3500} 0.177} & {\color[HTML]{53BF00} 0.718} & {\color[HTML]{4DC500} 0.091} & {\color[HTML]{4FC300} 0.042} & {\color[HTML]{3FD300} 0.207} & {\color[HTML]{D63C00} 0.683} & {\color[HTML]{4BC700} 0.075} & {\color[HTML]{47CB00} 0.052} & {\color[HTML]{3AD800} 0.214} & {\color[HTML]{D93900} 0.664} & {\color[HTML]{44CE00} 0.112} & {\color[HTML]{44CE00} 0.072} & {\color[HTML]{3AD800} 0.209} & {\color[HTML]{DC3600} 0.702} \\
phi4 & Calib-7 & {\color[HTML]{D83A00} 0.077} & {\color[HTML]{C94900} 0.069} & {\color[HTML]{E03200} 0.172} & {\color[HTML]{68AA00} 0.729} & {\color[HTML]{4BC700} 0.111} & {\color[HTML]{4AC800} 0.078} & {\color[HTML]{3DD500} 0.217} & {\color[HTML]{D43E00} 0.659} & {\color[HTML]{4BC700} 0.075} & {\color[HTML]{46CC00} 0.062} & {\color[HTML]{3BD700} 0.211} & {\color[HTML]{DA3800} 0.678} & {\color[HTML]{4CC600} 0.059} & {\color[HTML]{46CC00} 0.057} & {\color[HTML]{3DD500} 0.191} & {\color[HTML]{E03200} 0.736} \\
phi4 & Calib-5 + PS & {\color[HTML]{9F7300} 0.217} & {\color[HTML]{BF5300} 0.078} & {\color[HTML]{BB5700} 0.228} & {\color[HTML]{61B100} 0.725} & {\color[HTML]{45CD00} 0.151} & {\color[HTML]{4DC500} 0.053} & {\color[HTML]{3BD700} 0.235} & {\color[HTML]{D43E00} 0.659} & {\color[HTML]{41D100} 0.148} & {\color[HTML]{47CB00} 0.056} & {\color[HTML]{37DB00} 0.238} & {\color[HTML]{DA3800} 0.678} & {\color[HTML]{3BD700} 0.176} & {\color[HTML]{41D100} 0.091} & {\color[HTML]{37DB00} 0.231} & {\color[HTML]{E03200} 0.736} \\
phi4 & bce-auc  small  bert  is  7 & {\color[HTML]{D83A00} 0.077} & {\color[HTML]{C94900} 0.069} & {\color[HTML]{E03200} 0.172} & {\color[HTML]{68AA00} 0.729} & {\color[HTML]{4BC700} 0.11} & {\color[HTML]{4AC800} 0.078} & {\color[HTML]{3DD500} 0.217} & {\color[HTML]{D43E00} 0.66} & {\color[HTML]{4BC700} 0.073} & {\color[HTML]{46CC00} 0.059} & {\color[HTML]{3BD700} 0.21} & {\color[HTML]{DA3800} 0.679} & {\color[HTML]{4BC700} 0.062} & {\color[HTML]{46CC00} 0.057} & {\color[HTML]{3DD500} 0.191} & {\color[HTML]{E03200} 0.736} \\
phi4 & (auc)Calib-7 & {\color[HTML]{A46E00} 0.203} & {\color[HTML]{32E000} 0.205} & {\color[HTML]{AE6400} 0.248} & {\color[HTML]{44CE00} 0.71} & {\color[HTML]{34DE00} 0.275} & {\color[HTML]{32E000} 0.252} & {\color[HTML]{32E000} 0.305} & {\color[HTML]{D24000} 0.638} & {\color[HTML]{36DC00} 0.225} & {\color[HTML]{32E000} 0.203} & {\color[HTML]{32E000} 0.277} & {\color[HTML]{D93900} 0.664} & {\color[HTML]{35DD00} 0.221} & {\color[HTML]{32E000} 0.198} & {\color[HTML]{35DD00} 0.249} & {\color[HTML]{E03200} 0.742} \\
phi4 & (focal)Calib-7 & {\color[HTML]{DA3800} 0.072} & {\color[HTML]{C74B00} 0.071} & {\color[HTML]{DF3300} 0.173} & {\color[HTML]{59B900} 0.721} & {\color[HTML]{4CC600} 0.101} & {\color[HTML]{4BC700} 0.068} & {\color[HTML]{3ED400} 0.214} & {\color[HTML]{D43E00} 0.661} & {\color[HTML]{4DC500} 0.06} & {\color[HTML]{48CA00} 0.049} & {\color[HTML]{3BD700} 0.207} & {\color[HTML]{DA3800} 0.679} & {\color[HTML]{4CC600} 0.056} & {\color[HTML]{46CC00} 0.057} & {\color[HTML]{3DD500} 0.189} & {\color[HTML]{E03200} 0.74} \\
phi4 & auc  one  bert  is  1 & {\color[HTML]{AD6500} 0.181} & {\color[HTML]{60B200} 0.163} & {\color[HTML]{BD5500} 0.226} & {\color[HTML]{32E100} 0.7} & {\color[HTML]{42D000} 0.175} & {\color[HTML]{41D100} 0.142} & {\color[HTML]{3AD800} 0.244} & {\color[HTML]{D63C00} 0.674} & {\color[HTML]{40D200} 0.158} & {\color[HTML]{38DA00} 0.155} & {\color[HTML]{36DC00} 0.242} & {\color[HTML]{DA3800} 0.674} & {\color[HTML]{32E000} 0.247} & {\color[HTML]{37DB00} 0.16} & {\color[HTML]{32E000} 0.264} & {\color[HTML]{DE3400} 0.72} \\
phi4 & focal  one  bert  is  1 & {\color[HTML]{E13200} 0.056} & {\color[HTML]{E13200} 0.048} & {\color[HTML]{E13200} 0.171} & {\color[HTML]{46CC00} 0.711} & {\color[HTML]{51C100} 0.065} & {\color[HTML]{4FC300} 0.039} & {\color[HTML]{3FD300} 0.201} & {\color[HTML]{D73B00} 0.693} & {\color[HTML]{4EC400} 0.051} & {\color[HTML]{4BC700} 0.03} & {\color[HTML]{3BD700} 0.209} & {\color[HTML]{D93900} 0.664} & {\color[HTML]{48CA00} 0.086} & {\color[HTML]{46CC00} 0.06} & {\color[HTML]{3BD700} 0.202} & {\color[HTML]{DC3600} 0.702} \\
\hline
phi7 & LLM Prob. & {\color[HTML]{997900} 0.207} & {\color[HTML]{799900} 0.151} & {\color[HTML]{E03200} 0.245} & {\color[HTML]{E03200} 0.754} & {\color[HTML]{37DB00} 0.223} & {\color[HTML]{40D200} 0.15} & {\color[HTML]{39D900} 0.249} & {\color[HTML]{E03200} 0.758} & {\color[HTML]{32E000} 0.206} & {\color[HTML]{39D900} 0.152} & {\color[HTML]{32E000} 0.276} & {\color[HTML]{E03200} 0.66} & {\color[HTML]{46CC00} 0.105} & {\color[HTML]{4CC600} 0.049} & {\color[HTML]{38DA00} 0.23} & {\color[HTML]{DA3800} 0.639} \\
phi7 & LLM Prob + PS & {\color[HTML]{947E00} 0.216} & {\color[HTML]{D53D00} 0.067} & {\color[HTML]{E03200} 0.268} & {\color[HTML]{A27000} 0.713} & {\color[HTML]{3AD800} 0.205} & {\color[HTML]{47CB00} 0.103} & {\color[HTML]{39D900} 0.251} & {\color[HTML]{E03200} 0.757} & {\color[HTML]{3BD700} 0.144} & {\color[HTML]{48CA00} 0.052} & {\color[HTML]{35DD00} 0.253} & {\color[HTML]{E03200} 0.66} & {\color[HTML]{40D200} 0.147} & {\color[HTML]{4CC600} 0.05} & {\color[HTML]{35DD00} 0.251} & {\color[HTML]{DA3800} 0.639} \\
phi7 & verb  prob & {\color[HTML]{32E000} 0.403} & {\color[HTML]{967C00} 0.125} & {\color[HTML]{32E000} 28.697} & {\color[HTML]{918100} 0.702} & {\color[HTML]{E13200}     -} & {\color[HTML]{E13200}     -} & {\color[HTML]{E13200}     -} & {\color[HTML]{32E100}     -} & {\color[HTML]{E13200}     -} & {\color[HTML]{E13200}     -} & {\color[HTML]{E13200}     -} & {\color[HTML]{32E100}     -} & {\color[HTML]{E13200}     -} & {\color[HTML]{E13200}     -} & {\color[HTML]{E13200}     -} & {\color[HTML]{32E100}     -} \\
phi7 & Calib  -(cluster) & {\color[HTML]{C94900} 0.115} & {\color[HTML]{B35F00} 0.098} & {\color[HTML]{E03200} 0.221} & {\color[HTML]{848E00} 0.694} & {\color[HTML]{46CC00} 0.115} & {\color[HTML]{48CA00} 0.094} & {\color[HTML]{3CD600} 0.225} & {\color[HTML]{D83A00} 0.67} & {\color[HTML]{3FD300} 0.121} & {\color[HTML]{3DD500} 0.124} & {\color[HTML]{37DB00} 0.238} & {\color[HTML]{E03200} 0.659} & {\color[HTML]{42D000} 0.131} & {\color[HTML]{46CC00} 0.09} & {\color[HTML]{38DA00} 0.236} & {\color[HTML]{DB3700} 0.655} \\
phi7 & Calib  - & {\color[HTML]{D83A00} 0.088} & {\color[HTML]{D93900} 0.063} & {\color[HTML]{E03200} 0.22} & {\color[HTML]{4FC300} 0.659} & {\color[HTML]{4AC800} 0.088} & {\color[HTML]{4BC700} 0.072} & {\color[HTML]{3CD600} 0.227} & {\color[HTML]{D24000} 0.608} & {\color[HTML]{43CF00} 0.088} & {\color[HTML]{46CC00} 0.066} & {\color[HTML]{38DA00} 0.229} & {\color[HTML]{DE3400} 0.641} & {\color[HTML]{46CC00} 0.102} & {\color[HTML]{47CB00} 0.087} & {\color[HTML]{39D900} 0.227} & {\color[HTML]{DC3600} 0.659} \\
phi7 & Calib-7 & {\color[HTML]{C64C00} 0.122} & {\color[HTML]{CF4300} 0.072} & {\color[HTML]{E03200} 0.227} & {\color[HTML]{66AC00} 0.674} & {\color[HTML]{47CB00} 0.114} & {\color[HTML]{4AC800} 0.08} & {\color[HTML]{3CD600} 0.232} & {\color[HTML]{D53D00} 0.641} & {\color[HTML]{42D000} 0.1} & {\color[HTML]{46CC00} 0.065} & {\color[HTML]{38DA00} 0.228} & {\color[HTML]{E03200} 0.663} & {\color[HTML]{48CA00} 0.091} & {\color[HTML]{48CA00} 0.078} & {\color[HTML]{3AD800} 0.217} & {\color[HTML]{DF3300} 0.694} \\
phi7 & Calib-5 + PS & {\color[HTML]{BD5500} 0.139} & {\color[HTML]{D53D00} 0.067} & {\color[HTML]{E03200} 0.233} & {\color[HTML]{67AB00} 0.675} & {\color[HTML]{46CC00} 0.119} & {\color[HTML]{50C200} 0.036} & {\color[HTML]{3BD700} 0.236} & {\color[HTML]{D53D00} 0.641} & {\color[HTML]{40D200} 0.114} & {\color[HTML]{47CB00} 0.058} & {\color[HTML]{37DB00} 0.236} & {\color[HTML]{E03200} 0.663} & {\color[HTML]{44CE00} 0.115} & {\color[HTML]{49C900} 0.075} & {\color[HTML]{38DA00} 0.232} & {\color[HTML]{DF3300} 0.694} \\
phi7 & bce-auc  small  bert  is  7 & {\color[HTML]{C64C00} 0.122} & {\color[HTML]{CF4300} 0.072} & {\color[HTML]{E03200} 0.227} & {\color[HTML]{66AC00} 0.674} & {\color[HTML]{47CB00} 0.114} & {\color[HTML]{4AC800} 0.08} & {\color[HTML]{3CD600} 0.232} & {\color[HTML]{D53D00} 0.641} & {\color[HTML]{42D000} 0.099} & {\color[HTML]{46CC00} 0.065} & {\color[HTML]{38DA00} 0.228} & {\color[HTML]{E03200} 0.664} & {\color[HTML]{48CA00} 0.09} & {\color[HTML]{48CA00} 0.078} & {\color[HTML]{3AD800} 0.217} & {\color[HTML]{E03200} 0.695} \\
phi7 & (auc)Calib-7 & {\color[HTML]{8C8600} 0.232} & {\color[HTML]{32E000} 0.217} & {\color[HTML]{E03200} 0.281} & {\color[HTML]{4FC300} 0.659} & {\color[HTML]{32E000} 0.266} & {\color[HTML]{32E000} 0.256} & {\color[HTML]{32E000} 0.307} & {\color[HTML]{D33F00} 0.624} & {\color[HTML]{32E000} 0.207} & {\color[HTML]{32E000} 0.205} & {\color[HTML]{32E000} 0.274} & {\color[HTML]{DF3300} 0.649} & {\color[HTML]{32E000} 0.25} & {\color[HTML]{32E000} 0.238} & {\color[HTML]{32E000} 0.28} & {\color[HTML]{E03200} 0.704} \\
phi7 & (focal)Calib-7 & {\color[HTML]{C54D00} 0.124} & {\color[HTML]{CF4300} 0.072} & {\color[HTML]{E03200} 0.228} & {\color[HTML]{5BB700} 0.667} & {\color[HTML]{48CA00} 0.104} & {\color[HTML]{49C900} 0.09} & {\color[HTML]{3CD600} 0.231} & {\color[HTML]{D43E00} 0.633} & {\color[HTML]{42D000} 0.097} & {\color[HTML]{48CA00} 0.05} & {\color[HTML]{38DA00} 0.228} & {\color[HTML]{E03200} 0.657} & {\color[HTML]{49C900} 0.079} & {\color[HTML]{4AC800} 0.067} & {\color[HTML]{3AD800} 0.215} & {\color[HTML]{E03200} 0.698} \\
phi7 & auc  one  bert  is  1 & {\color[HTML]{A07200} 0.193} & {\color[HTML]{4BC700} 0.194} & {\color[HTML]{E03200} 0.264} & {\color[HTML]{32E100} 0.64} & {\color[HTML]{37DB00} 0.228} & {\color[HTML]{35DD00} 0.228} & {\color[HTML]{34DE00} 0.287} & {\color[HTML]{D14100} 0.603} & {\color[HTML]{32E000} 0.212} & {\color[HTML]{32E000} 0.206} & {\color[HTML]{32E000} 0.277} & {\color[HTML]{DD3500} 0.63} & {\color[HTML]{3CD600} 0.175} & {\color[HTML]{3CD600} 0.164} & {\color[HTML]{35DD00} 0.258} & {\color[HTML]{DC3600} 0.659} \\
phi7 & focal  one  bert  is  1 & {\color[HTML]{E13200} 0.071} & {\color[HTML]{E13200} 0.056} & {\color[HTML]{E13200} 0.218} & {\color[HTML]{44CE00} 0.652} & {\color[HTML]{4EC400} 0.06} & {\color[HTML]{4DC500} 0.059} & {\color[HTML]{3DD500} 0.223} & {\color[HTML]{D24000} 0.61} & {\color[HTML]{47CB00} 0.064} & {\color[HTML]{47CB00} 0.056} & {\color[HTML]{38DA00} 0.226} & {\color[HTML]{DF3300} 0.648} & {\color[HTML]{48CA00} 0.09} & {\color[HTML]{49C900} 0.071} & {\color[HTML]{39D900} 0.223} & {\color[HTML]{DC3600} 0.662} \\
\hline

==> tables/text/small_top_3_reults_text.tex <==
llama31-8 & LLM Prob. & {\color[HTML]{32E000} 0.316} & {\color[HTML]{6EA400} 0.163} & {\color[HTML]{32E000} 0.333} & {\color[HTML]{32E100} 0.651} & {\color[HTML]{7E9400} 0.16} & {\color[HTML]{E13200} 0.048} & {\color[HTML]{5CB600} 0.242} & {\color[HTML]{32E100} 0.693} & {\color[HTML]{6EA400} 0.183} & {\color[HTML]{957D00} 0.123} & {\color[HTML]{5DB500} 0.247} & {\color[HTML]{5EB400} 0.718} & {\color[HTML]{32E000} 0.505} & {\color[HTML]{769C00} 0.137} & {\color[HTML]{32E000} 0.47} & {\color[HTML]{32E100} 0.645} \\
llama31-8 & LLM Prob + PS & {\color[HTML]{739F00} 0.226} & {\color[HTML]{DE3400} 0.052} & {\color[HTML]{739F00} 0.281} & {\color[HTML]{32E100} 0.651} & {\color[HTML]{6BA700} 0.177} & {\color[HTML]{D53D00} 0.059} & {\color[HTML]{32E000} 0.256} & {\color[HTML]{34DE00} 0.694} & {\color[HTML]{32E000} 0.231} & {\color[HTML]{A66C00} 0.109} & {\color[HTML]{54BE00} 0.25} & {\color[HTML]{E03200} 0.773} & {\color[HTML]{987A00} 0.265} & {\color[HTML]{E13200} 0.037} & {\color[HTML]{B65C00} 0.26} & {\color[HTML]{E03200} 0.708} \\
llama31-8 & Calib-1 & {\color[HTML]{DE3400} 0.081} & {\color[HTML]{D43E00} 0.062} & {\color[HTML]{E13200} 0.195} & {\color[HTML]{E03200} 0.754} & {\color[HTML]{CB4700} 0.09} & {\color[HTML]{CC4600} 0.067} & {\color[HTML]{BF5300} 0.21} & {\color[HTML]{6FA300} 0.714} & {\color[HTML]{D53D00} 0.101} & {\color[HTML]{B85A00} 0.095} & {\color[HTML]{CF4300} 0.207} & {\color[HTML]{32E100} 0.699} & {\color[HTML]{DA3800} 0.11} & {\color[HTML]{B26000} 0.081} & {\color[HTML]{DC3600} 0.199} & {\color[HTML]{AC6600} 0.689} \\
llama31-8 & Calib-1(cluster) & {\color[HTML]{D04200} 0.1} & {\color[HTML]{CA4800} 0.072} & {\color[HTML]{C74B00} 0.215} & {\color[HTML]{A36F00} 0.718} & {\color[HTML]{B45E00} 0.111} & {\color[HTML]{C84A00} 0.071} & {\color[HTML]{977B00} 0.223} & {\color[HTML]{57BB00} 0.706} & {\color[HTML]{C54D00} 0.114} & {\color[HTML]{CE4400} 0.077} & {\color[HTML]{CA4800} 0.209} & {\color[HTML]{42D000} 0.706} & {\color[HTML]{D93900} 0.112} & {\color[HTML]{BC5600} 0.071} & {\color[HTML]{DC3600} 0.199} & {\color[HTML]{C25000} 0.697} \\
llama31-8 & Calib-7 & {\color[HTML]{E03200} 0.078} & {\color[HTML]{E13200} 0.05} & {\color[HTML]{DB3700} 0.199} & {\color[HTML]{D53D00} 0.747} & {\color[HTML]{DE3400} 0.072} & {\color[HTML]{D93900} 0.055} & {\color[HTML]{DA3800} 0.201} & {\color[HTML]{C34F00} 0.743} & {\color[HTML]{D53D00} 0.101} & {\color[HTML]{DF3300} 0.063} & {\color[HTML]{DB3700} 0.203} & {\color[HTML]{55BD00} 0.714} & {\color[HTML]{DD3500} 0.104} & {\color[HTML]{AE6400} 0.084} & {\color[HTML]{E03200} 0.193} & {\color[HTML]{D33F00} 0.703} \\
llama31-8 & Calib-5 + PS & {\color[HTML]{A76B00} 0.156} & {\color[HTML]{9C7600} 0.118} & {\color[HTML]{A96900} 0.239} & {\color[HTML]{D53D00} 0.747} & {\color[HTML]{A56D00} 0.124} & {\color[HTML]{8C8600} 0.128} & {\color[HTML]{8B8700} 0.227} & {\color[HTML]{C34F00} 0.743} & {\color[HTML]{7B9700} 0.173} & {\color[HTML]{C94900} 0.081} & {\color[HTML]{7C9600} 0.236} & {\color[HTML]{55BD00} 0.714} & {\color[HTML]{BA5800} 0.186} & {\color[HTML]{C84A00} 0.06} & {\color[HTML]{C94900} 0.229} & {\color[HTML]{D33F00} 0.703} \\
llama31-8 & (focal)Calib-7 & {\color[HTML]{D83A00} 0.088} & {\color[HTML]{DA3800} 0.056} & {\color[HTML]{DB3700} 0.199} & {\color[HTML]{CC4600} 0.742} & {\color[HTML]{E13200} 0.07} & {\color[HTML]{DD3500} 0.051} & {\color[HTML]{DA3800} 0.201} & {\color[HTML]{C05200} 0.742} & {\color[HTML]{E13200} 0.092} & {\color[HTML]{D93900} 0.068} & {\color[HTML]{E13200} 0.201} & {\color[HTML]{49C900} 0.709} & {\color[HTML]{E13200} 0.095} & {\color[HTML]{B45E00} 0.079} & {\color[HTML]{E13200} 0.192} & {\color[HTML]{C25000} 0.697} \\
llama31-8 & (bce:auc)Calib-7 & {\color[HTML]{E13200} 0.077} & {\color[HTML]{DE3400} 0.052} & {\color[HTML]{DB3700} 0.199} & {\color[HTML]{D33F00} 0.746} & {\color[HTML]{DE3400} 0.072} & {\color[HTML]{D93900} 0.055} & {\color[HTML]{DA3800} 0.201} & {\color[HTML]{C34F00} 0.743} & {\color[HTML]{D63C00} 0.1} & {\color[HTML]{E13200} 0.062} & {\color[HTML]{DB3700} 0.203} & {\color[HTML]{53BF00} 0.713} & {\color[HTML]{DD3500} 0.104} & {\color[HTML]{AE6400} 0.084} & {\color[HTML]{E03200} 0.193} & {\color[HTML]{D33F00} 0.703} \\
llama31-8 & (auc)Calib-7 & {\color[HTML]{65AD00} 0.246} & {\color[HTML]{32E000} 0.223} & {\color[HTML]{72A000} 0.282} & {\color[HTML]{61B100} 0.679} & {\color[HTML]{32E000} 0.23} & {\color[HTML]{32E000} 0.214} & {\color[HTML]{41D100} 0.251} & {\color[HTML]{E03200} 0.753} & {\color[HTML]{50C200} 0.207} & {\color[HTML]{32E000} 0.203} & {\color[HTML]{32E000} 0.262} & {\color[HTML]{3DD500} 0.704} & {\color[HTML]{B26000} 0.204} & {\color[HTML]{32E000} 0.201} & {\color[HTML]{B95900} 0.254} & {\color[HTML]{BA5800} 0.694} \\
llama31-8 & Calib-t3 & {\color[HTML]{DF3300} 0.079} & {\color[HTML]{D24000} 0.064} & {\color[HTML]{DD3500} 0.198} & {\color[HTML]{DA3800} 0.75} & {\color[HTML]{DC3600} 0.074} & {\color[HTML]{C44E00} 0.075} & {\color[HTML]{E13200} 0.199} & {\color[HTML]{D24000} 0.748} & {\color[HTML]{DF3300} 0.093} & {\color[HTML]{C94900} 0.081} & {\color[HTML]{D53D00} 0.205} & {\color[HTML]{42D000} 0.706} & {\color[HTML]{DE3400} 0.101} & {\color[HTML]{AB6700} 0.087} & {\color[HTML]{DF3300} 0.194} & {\color[HTML]{CA4800} 0.7} \\
\hline
gemma9 & LLM Prob. & {\color[HTML]{32E000} 0.251} & {\color[HTML]{66AC00} 0.175} & {\color[HTML]{32E000} 0.291} & {\color[HTML]{DD3500} 0.668} & {\color[HTML]{68AA00} 0.187} & {\color[HTML]{70A200} 0.161} & {\color[HTML]{32E000} 0.266} & {\color[HTML]{32E100} 0.604} & {\color[HTML]{32E000} 0.293} & {\color[HTML]{55BD00} 0.179} & {\color[HTML]{32E000} 0.293} & {\color[HTML]{E03200} 0.757} & {\color[HTML]{32E000} 0.444} & {\color[HTML]{779B00} 0.142} & {\color[HTML]{32E000} 0.42} & {\color[HTML]{E03200} 0.691} \\
gemma9 & LLM Prob + PS & {\color[HTML]{A56D00} 0.137} & {\color[HTML]{D04200} 0.065} & {\color[HTML]{B16100} 0.246} & {\color[HTML]{E03200} 0.669} & {\color[HTML]{C15100} 0.107} & {\color[HTML]{E13200} 0.034} & {\color[HTML]{898900} 0.236} & {\color[HTML]{32E100} 0.604} & {\color[HTML]{7C9600} 0.206} & {\color[HTML]{9E7400} 0.102} & {\color[HTML]{997900} 0.254} & {\color[HTML]{E03200} 0.757} & {\color[HTML]{B85A00} 0.184} & {\color[HTML]{DF3300} 0.046} & {\color[HTML]{C25000} 0.261} & {\color[HTML]{E03200} 0.691} \\
gemma9 & Calib-1 & {\color[HTML]{E13200} 0.079} & {\color[HTML]{E13200} 0.048} & {\color[HTML]{D24000} 0.234} & {\color[HTML]{32E100} 0.618} & {\color[HTML]{CB4700} 0.098} & {\color[HTML]{AE6400} 0.091} & {\color[HTML]{D24000} 0.211} & {\color[HTML]{C15100} 0.694} & {\color[HTML]{E13200} 0.089} & {\color[HTML]{C84A00} 0.058} & {\color[HTML]{E13200} 0.227} & {\color[HTML]{32E100} 0.626} & {\color[HTML]{E13200} 0.105} & {\color[HTML]{C94900} 0.067} & {\color[HTML]{E13200} 0.228} & {\color[HTML]{32E100} 0.613} \\
gemma9 & Calib-1(cluster) & {\color[HTML]{957D00} 0.153} & {\color[HTML]{977B00} 0.124} & {\color[HTML]{977B00} 0.255} & {\color[HTML]{62B000} 0.632} & {\color[HTML]{B26000} 0.121} & {\color[HTML]{A86A00} 0.098} & {\color[HTML]{A96900} 0.225} & {\color[HTML]{A17100} 0.674} & {\color[HTML]{BD5500} 0.13} & {\color[HTML]{9E7400} 0.102} & {\color[HTML]{CB4700} 0.235} & {\color[HTML]{4EC400} 0.647} & {\color[HTML]{D04200} 0.137} & {\color[HTML]{987A00} 0.112} & {\color[HTML]{DE3400} 0.231} & {\color[HTML]{858D00} 0.65} \\
gemma9 & Calib-7 & {\color[HTML]{C54D00} 0.106} & {\color[HTML]{CF4300} 0.066} & {\color[HTML]{D04200} 0.235} & {\color[HTML]{848E00} 0.642} & {\color[HTML]{DD3500} 0.082} & {\color[HTML]{BD5500} 0.074} & {\color[HTML]{E13200} 0.206} & {\color[HTML]{DC3600} 0.711} & {\color[HTML]{B65C00} 0.139} & {\color[HTML]{BB5700} 0.072} & {\color[HTML]{C34F00} 0.238} & {\color[HTML]{56BC00} 0.653} & {\color[HTML]{C64C00} 0.157} & {\color[HTML]{C05200} 0.075} & {\color[HTML]{D24000} 0.244} & {\color[HTML]{6CA600} 0.639} \\
gemma9 & Calib-5 + PS & {\color[HTML]{DD3500} 0.082} & {\color[HTML]{DF3300} 0.05} & {\color[HTML]{D53D00} 0.233} & {\color[HTML]{848E00} 0.642} & {\color[HTML]{D33F00} 0.091} & {\color[HTML]{B75B00} 0.081} & {\color[HTML]{BB5700} 0.219} & {\color[HTML]{DC3600} 0.711} & {\color[HTML]{DA3800} 0.096} & {\color[HTML]{E13200} 0.032} & {\color[HTML]{D63C00} 0.231} & {\color[HTML]{56BC00} 0.653} & {\color[HTML]{DE3400} 0.11} & {\color[HTML]{E13200} 0.045} & {\color[HTML]{E13200} 0.228} & {\color[HTML]{6CA600} 0.639} \\
gemma9 & (focal)Calib-7 & {\color[HTML]{CC4600} 0.099} & {\color[HTML]{E03200} 0.049} & {\color[HTML]{D24000} 0.234} & {\color[HTML]{7D9500} 0.64} & {\color[HTML]{DC3600} 0.083} & {\color[HTML]{BE5400} 0.073} & {\color[HTML]{DE3400} 0.207} & {\color[HTML]{D93900} 0.709} & {\color[HTML]{C64C00} 0.12} & {\color[HTML]{B85A00} 0.075} & {\color[HTML]{CE4400} 0.234} & {\color[HTML]{56BC00} 0.653} & {\color[HTML]{CD4500} 0.142} & {\color[HTML]{CA4800} 0.066} & {\color[HTML]{D53D00} 0.241} & {\color[HTML]{5EB400} 0.633} \\
gemma9 & (bce:auc)Calib-7 & {\color[HTML]{C54D00} 0.106} & {\color[HTML]{CE4400} 0.067} & {\color[HTML]{CD4500} 0.236} & {\color[HTML]{809200} 0.641} & {\color[HTML]{DD3500} 0.082} & {\color[HTML]{BC5600} 0.075} & {\color[HTML]{E13200} 0.206} & {\color[HTML]{DC3600} 0.711} & {\color[HTML]{B75B00} 0.137} & {\color[HTML]{BC5600} 0.071} & {\color[HTML]{C64C00} 0.237} & {\color[HTML]{56BC00} 0.653} & {\color[HTML]{C64C00} 0.157} & {\color[HTML]{C05200} 0.075} & {\color[HTML]{D24000} 0.244} & {\color[HTML]{6CA600} 0.639} \\
gemma9 & (auc)Calib-7 & {\color[HTML]{4AC800} 0.227} & {\color[HTML]{32E000} 0.229} & {\color[HTML]{40D200} 0.286} & {\color[HTML]{35DD00} 0.619} & {\color[HTML]{32E000} 0.236} & {\color[HTML]{32E000} 0.231} & {\color[HTML]{43CF00} 0.26} & {\color[HTML]{E03200} 0.714} & {\color[HTML]{62B000} 0.237} & {\color[HTML]{32E000} 0.217} & {\color[HTML]{41D100} 0.287} & {\color[HTML]{4BC700} 0.645} & {\color[HTML]{997900} 0.243} & {\color[HTML]{32E000} 0.206} & {\color[HTML]{A66C00} 0.292} & {\color[HTML]{4AC800} 0.624} \\
gemma9 & Calib-t3 & {\color[HTML]{D63C00} 0.089} & {\color[HTML]{C74B00} 0.074} & {\color[HTML]{E13200} 0.229} & {\color[HTML]{A36F00} 0.651} & {\color[HTML]{E13200} 0.079} & {\color[HTML]{B95900} 0.078} & {\color[HTML]{E13200} 0.206} & {\color[HTML]{D73B00} 0.708} & {\color[HTML]{CA4800} 0.115} & {\color[HTML]{AE6400} 0.085} & {\color[HTML]{D33F00} 0.232} & {\color[HTML]{4CC600} 0.646} & {\color[HTML]{D53D00} 0.128} & {\color[HTML]{AA6800} 0.095} & {\color[HTML]{DA3800} 0.235} & {\color[HTML]{5AB800} 0.631} \\
\hline
phi7 & LLM Prob. & {\color[HTML]{33DF00} 0.206} & {\color[HTML]{6DA500} 0.152} & {\color[HTML]{32E000} 0.276} & {\color[HTML]{C25000} 0.66} & {\color[HTML]{C64C00} 0.105} & {\color[HTML]{E13200} 0.049} & {\color[HTML]{B85A00} 0.23} & {\color[HTML]{32E100} 0.639} & {\color[HTML]{5CB600} 0.223} & {\color[HTML]{868C00} 0.15} & {\color[HTML]{AD6500} 0.249} & {\color[HTML]{E03200} 0.758} & {\color[HTML]{32E000} 0.414} & {\color[HTML]{8A8800} 0.131} & {\color[HTML]{32E000} 29.197} & {\color[HTML]{957D00} 0.686} \\
phi7 & LLM Prob + PS & {\color[HTML]{8A8800} 0.144} & {\color[HTML]{DE3400} 0.052} & {\color[HTML]{848E00} 0.253} & {\color[HTML]{C25000} 0.66} & {\color[HTML]{9B7700} 0.147} & {\color[HTML]{E03200} 0.05} & {\color[HTML]{809200} 0.251} & {\color[HTML]{32E100} 0.639} & {\color[HTML]{6DA500} 0.205} & {\color[HTML]{AB6700} 0.103} & {\color[HTML]{A96900} 0.251} & {\color[HTML]{DF3300} 0.757} & {\color[HTML]{9B7700} 0.228} & {\color[HTML]{E13200} 0.044} & {\color[HTML]{E03200} 0.271} & {\color[HTML]{E03200} 0.702} \\
phi7 & Calib-1 & {\color[HTML]{D83A00} 0.088} & {\color[HTML]{CE4400} 0.066} & {\color[HTML]{D93900} 0.229} & {\color[HTML]{32E100} 0.641} & {\color[HTML]{C94900} 0.102} & {\color[HTML]{BD5500} 0.087} & {\color[HTML]{C05200} 0.227} & {\color[HTML]{67AB00} 0.659} & {\color[HTML]{E13200} 0.088} & {\color[HTML]{C44E00} 0.072} & {\color[HTML]{DC3600} 0.227} & {\color[HTML]{32E100} 0.608} & {\color[HTML]{E13200} 0.104} & {\color[HTML]{B85A00} 0.085} & {\color[HTML]{E03200} 0.221} & {\color[HTML]{32E100} 0.665} \\
phi7 & Calib-1(cluster) & {\color[HTML]{AA6800} 0.121} & {\color[HTML]{8D8500} 0.124} & {\color[HTML]{B95900} 0.238} & {\color[HTML]{BA5800} 0.659} & {\color[HTML]{AB6700} 0.131} & {\color[HTML]{BB5700} 0.09} & {\color[HTML]{A86A00} 0.236} & {\color[HTML]{5DB500} 0.655} & {\color[HTML]{C64C00} 0.115} & {\color[HTML]{B26000} 0.094} & {\color[HTML]{E13200} 0.225} & {\color[HTML]{7A9800} 0.67} & {\color[HTML]{DF3300} 0.107} & {\color[HTML]{B65C00} 0.087} & {\color[HTML]{E13200} 0.215} & {\color[HTML]{DC3600} 0.701} \\
phi7 & Calib-7 & {\color[HTML]{C74B00} 0.1} & {\color[HTML]{D04200} 0.065} & {\color[HTML]{DD3500} 0.228} & {\color[HTML]{D93900} 0.663} & {\color[HTML]{D43E00} 0.091} & {\color[HTML]{C64C00} 0.078} & {\color[HTML]{DB3700} 0.217} & {\color[HTML]{C64C00} 0.694} & {\color[HTML]{C74B00} 0.114} & {\color[HTML]{BE5400} 0.08} & {\color[HTML]{D24000} 0.232} & {\color[HTML]{58BA00} 0.641} & {\color[HTML]{D53D00} 0.125} & {\color[HTML]{BC5600} 0.081} & {\color[HTML]{E03200} 0.225} & {\color[HTML]{5CB600} 0.674} \\
phi7 & Calib-5 + PS & {\color[HTML]{B45E00} 0.114} & {\color[HTML]{D73B00} 0.058} & {\color[HTML]{C05200} 0.236} & {\color[HTML]{D93900} 0.663} & {\color[HTML]{BC5600} 0.115} & {\color[HTML]{C84A00} 0.075} & {\color[HTML]{B35F00} 0.232} & {\color[HTML]{C64C00} 0.694} & {\color[HTML]{C25000} 0.119} & {\color[HTML]{E13200} 0.036} & {\color[HTML]{C94900} 0.236} & {\color[HTML]{58BA00} 0.641} & {\color[HTML]{CA4800} 0.143} & {\color[HTML]{CD4500} 0.064} & {\color[HTML]{E03200} 0.233} & {\color[HTML]{5CB600} 0.674} \\
phi7 & (focal)Calib-7 & {\color[HTML]{CC4600} 0.097} & {\color[HTML]{E13200} 0.05} & {\color[HTML]{DD3500} 0.228} & {\color[HTML]{AB6700} 0.657} & {\color[HTML]{E13200} 0.079} & {\color[HTML]{D04200} 0.067} & {\color[HTML]{E13200} 0.215} & {\color[HTML]{D04200} 0.698} & {\color[HTML]{D14100} 0.104} & {\color[HTML]{B65C00} 0.09} & {\color[HTML]{D43E00} 0.231} & {\color[HTML]{4FC300} 0.633} & {\color[HTML]{DB3700} 0.114} & {\color[HTML]{BF5300} 0.078} & {\color[HTML]{E03200} 0.224} & {\color[HTML]{3BD700} 0.667} \\
phi7 & (bce:auc)Calib-7 & {\color[HTML]{C74B00} 0.1} & {\color[HTML]{D14100} 0.064} & {\color[HTML]{DD3500} 0.228} & {\color[HTML]{E03200} 0.664} & {\color[HTML]{D43E00} 0.091} & {\color[HTML]{C64C00} 0.078} & {\color[HTML]{DB3700} 0.217} & {\color[HTML]{C64C00} 0.694} & {\color[HTML]{C74B00} 0.114} & {\color[HTML]{BE5400} 0.08} & {\color[HTML]{D24000} 0.232} & {\color[HTML]{58BA00} 0.641} & {\color[HTML]{D53D00} 0.125} & {\color[HTML]{BC5600} 0.081} & {\color[HTML]{E03200} 0.225} & {\color[HTML]{5CB600} 0.674} \\
phi7 & (auc)Calib-7 & {\color[HTML]{32E000} 0.207} & {\color[HTML]{32E000} 0.205} & {\color[HTML]{39D900} 0.274} & {\color[HTML]{6EA400} 0.649} & {\color[HTML]{32E000} 0.25} & {\color[HTML]{32E000} 0.238} & {\color[HTML]{32E000} 0.28} & {\color[HTML]{E03200} 0.704} & {\color[HTML]{32E000} 0.266} & {\color[HTML]{32E000} 0.256} & {\color[HTML]{32E000} 0.307} & {\color[HTML]{44CE00} 0.624} & {\color[HTML]{987A00} 0.233} & {\color[HTML]{32E000} 0.221} & {\color[HTML]{E03200} 0.282} & {\color[HTML]{49C900} 0.67} \\
phi7 & Calib-t3 & {\color[HTML]{E13200} 0.082} & {\color[HTML]{D24000} 0.063} & {\color[HTML]{E13200} 0.227} & {\color[HTML]{B35F00} 0.658} & {\color[HTML]{CC4600} 0.099} & {\color[HTML]{B26000} 0.099} & {\color[HTML]{D33F00} 0.22} & {\color[HTML]{B06200} 0.686} & {\color[HTML]{C44E00} 0.117} & {\color[HTML]{A96900} 0.106} & {\color[HTML]{CF4300} 0.233} & {\color[HTML]{45CD00} 0.625} & {\color[HTML]{DF3300} 0.106} & {\color[HTML]{B95900} 0.084} & {\color[HTML]{E03200} 0.22} & {\color[HTML]{61B100} 0.675} \\
\hline

